Substring Density Estimation from Traces

In the trace reconstruction problem, one seeks to reconstruct a binary string $s$ from a collection of traces, each of which is obtained by passing $s$ through a deletion channel. It is known that $\exp(\tilde O(n^{1/5}))$ traces suffice to reconstruct any length-$n$ string with high probability. We consider a variant of the trace reconstruction problem where the goal is to recover a "density map" that indicates the locations of each length-$k$ substring throughout $s$. We show that $\epsilon^{-2}\cdot \text{poly}(n)$ traces suffice to recover the density map with error at most $\epsilon$. As a result, when restricted to a set of source strings whose minimum "density map distance" is at least $1/\text{poly}(n)$, the trace reconstruction problem can be solved with polynomially many traces.

==> intro06-27.tex <==
% !TEX root = main.tex


In the trace reconstruction problem, there is an unknown binary string $s \in \{0,1\}^n$, which we wish to reconstruct based on $T$ subsequences (or traces) of $s$.
Each trace is obtained by passing the {\it source string} $s$ through a deletion channel, which deletes each bit of $s$  independently with probability $p$.
The main question of interest is how many traces are needed in order to reconstruct $s$ correctly.

This problem was originally proposed by Batu et al.~\cite{Batu}, motivated by problems in sequence alignment, phylogeny, and computational biology~\cite{Pfevzner}.
% Since then, it received considerable attention from several perspectives~\cite{}.
% This problem received considerable attention in recent years~\cite{abroshan2019coding,magner2016fundamental,mao2018models,holenstein2008trace,de2017optimal,hartung2018trace,nazarov2017trace,srinivasavaradhan2018maximum,srinivasavaradhan2019symbolwise,}, partially due to 
% the fact that DNA sequencing technologies 
% % and  especially nanopore sequencing technologies 
% suffer from deletion errors~\cite{mao2018models}.
% In addition, the trace reconstruction problem has applications in immunogenomics, where one seeks to reconstruct the set of germline genes of an individual by analyzing antibody repertoires.
% In this setting, each antibody can be viewed as a trace generated by recombining elements from the germline genes \cite{bhardwaj2020trace}.
Most of the work on the trace reconstruction problem has focused on characterizing the minimum number of traces needed for reconstructing the source string $s$ exactly.
The most common formulation of the problem, known as
% Two important formulations of this problem are the
\emph{worst-case trace reconstruction}~\cite{Servedio}, 
requires the reconstruction algorithm to recover $s \in \{0,1\}^n$ exactly with high probability as $n \to \infty$ for \emph{any} string $s \in \{0,1\}^n$.
While this problem has received considerable attention, there is still a significant gap between upper and lower bounds on the number of traces needed.
Currently, the best lower bound
% , due to Chase, 
is $\tilde{\Omega}(n^{3/2})$, while the best upper bound
% , due to Chase, 
is $\exp(\tilde{O}(n^{1/5}))$, both due to Chase~\cite{Chase2,Chase}.

Several different formulations have been proposed to avoid the worst-case assumption and allow the derivation of significantly better upper bounds.
For example, in the average-case formulation, $s$ is assumed to be drawn uniformly at random from all $\{0,1\}^n$ strings, in which case $T = \exp(O(\log^{1/3}(n)))$ traces are sufficient \cite{Peres2}.
Moreover, an approximate trace reconstruction problem has also been formulated, where a fraction of the recovered bits is allowed to be incorrect~\cite{Davies}, and the problem of finding the maximum likelihood $s$ from a small number of traces $T$ (possibly insufficient for exact reconstruction) has also been considered~\cite{Diggavi}.
The problem has also been considered in the smoothed complexity model~\cite{Servedio2}, in which a worst-case string is passed through a binary symmetric channel before trace generation, and the noise-corrupted string needs to be reconstructed with high probability (recall that a binary symmetric channel flips each bit in the string independently with some fixed probability). 


The current best upper bounds for worst-case trace reconstruction \cite{Peres,Servedio,Chase} are obtained using algorithms that consider each pair of possible source strings $x, y$, and decide whether the set of traces looks more like a set of traces from $x$, or more like a set of traces from $y$ (we formalize this shortly).  
Then if there are enough traces, with high probability the true source string $s$ will be the unique string $u$ such that the set of traces looks more like it came from $u$ than 
from any other string in $\{0, 1\}^n$.  
Therefore, the trace reconstruction problem is closely related to the string distinguishing problem \cite{Sudan,Bruck} \iscomment{is this the name of the problem?}, where 
% given the source string is either $x \in \{0, 1\}^n$ or $y \in \{0, 1\}^n$, 
we want to decide from the set of traces whether the source string is either $x \in \{0, 1\}^n$ or $y \in \{0, 1\}^n$ with high probability.  
The best existing upper bound of $\exp(O(n^{1/5}))$ for worst-case trace reconstruction \cite{Chase} is proved using the fact that any two strings can be distinguished using $\exp(O(n^{1/5}))$ traces.
It has also been shown that string pairs at constant Hamming distance can be distinguished using $\text{poly}(n)$ traces \cite{Mcgregor,Sudan}, and strings at constant Levenshtein distance can be distinguished using $\text{poly}(n)$ traces \cite{Bruck}.  



To distinguish between two strings $x$ and $y$ from a set of traces, current algorithms identify a function $f_{x,y}$ such that $\Vert E[f_{x,y}(\tilde{X})] - E[f_{x,y}(\tilde{Y})] \Vert$ is sufficiently large where $\tilde{X}$ denotes a trace of $x$ and $\Vert \cdot \Vert$ denotes a norm.  
Given $T$ traces $\tilde{S}_1,\dots, \tilde{S}_T$ of a source string $s$, $E[f_{x,y}(\tilde{S})]$ is estimated as $\frac{1}{T} \sum_{i=1}^T f_{x,y}(\tilde{S}_i)$ and we say that $x$ {\it beats} $y$ if $\frac{1}{T} \sum_{i=1}^T f_{x,y}(\tilde{S}_i)$ is closer to $E[f_{x,y}(\tilde{X})]$ than to $E[f_{x,y}(\tilde{Y})]$. 
Observe that if $f_{x, y}$ is such that $\Vert E[f_{x,y}(\tilde{X})] - E[f_{x,y}(\tilde{Y})] \Vert$ is large enough, then assuming the source string is $x$ or $y$, we can distinguish between the two cases given a reasonable number of traces.
If there is a unique string $u$ such that $u$ beats all other strings, then $u$ is output as the reconstruction.  
Using concentration inequalities, one can show that with enough traces, the true string $s$ will be the unique string that beats all other strings, and will therefore be reconstructed correctly with high probability.   

% Observe that if $f_{x, y}$ is such that $|E[f_{x,y}(\tilde{X})] - E[f_{x,y}(\tilde{Y})]|$ is large enough, then assuming the source string is $x$ or $y$, we can distinguish between the two cases given a reasonable number of traces.
% If we can do this reliably enough for each string pair $x, y$, then we will be able to reconstruct the source string by finding the unbeaten string $z$.
% Therefore, the worst-case trace reconstruction problem is equivalent in a sense to the problem of distinguishing whether traces came from one string or another.  
% The challenge with the methodology for trace reconstruction describes above is finding a function $f_{x, y}$ such that $|E[f_{x,y}(\tilde{X})] - E[f_{x,y}(\tilde{Y})]|$ is large enough for each string pair $x, y$ so that $x$ can be distinguished from $y$ with high probability given a reasonable number of traces.

The first such measure $f_{x,y}$ introduced in \cite{Servedio,Peres} is simply the value of a single bit in the trace, i.e., $f_{x,y}(\tilde{S}) = \tilde{S}_i$ for source string $s$ and some index $i$ that depends on $x$ and $y$, and the norm used for measuring distance is absolute value.
This is known in the literature as a single bit statistic, and was used to obtain an upper bound of $\exp{(O(n^{1/3}))}$ traces.
The current best upper bound \cite{Chase} picks a more complicated function $f_{x,y}$ that involves multiple bits, and yields an upper bound of  $\exp{(O(n^{1/5}))}$.
A choice of $f_{x,y}$ that uses multiple bits in combination is known in the literature as a multi-bit statistic.

Furthermore, obtaining lower bounds for the number of traces needed in the trace reconstruction problem amounts to proving a lower bound on the number of traces required to distinguish two strings since any algorithm to solve the trace reconstruction problem can be used to solve the string distinguishing problem.
For a string $a$, let $a^i$ denote the string where $a$ is repeated $i$ times.  
The current best lower bound of $\tilde{\Omega}(n^{3/2})$ for trace reconstruction is obtained by analyzing the string pair $(01)^{k} 1 (01)^{k+1} $ and $(01)^{k+1} 1 (01)^{k}$ where $n = 2k+3$.

Another important structure in trace reconstruction and sequence reconstruction problems in general is the $k$-deck of a sequence.  The $k$-deck of a sequence $s \in \{0,1\}^n$ is the multiset of all length-$k$ substrings, formally defined as
\al{
\cS_k(s) = \{ s[i:i+k-1] : i =1,\dots,n-k+1 \}.
}
In the bioinformatics community, the $k$-deck is known as the $k$-spectrum, and each length $k$ substring is called a $k$-mer.  
Most practical DNA reconstruction algorithms are given as input a set of substrings (termed reads) of the DNA sequence that are potentially affected by substitutions.  
With enough reads, the DNA sequencing problem is therefore equivalent to reconstructing the sequence from a (potentially noisy) version of the $k$-deck where $k$ is the read length.
Given an approximation of the $k$-deck, a debruijn graph is formed, where each node corresponds to a $k$-mer, and there is a directed edge from node $u$ to node $v$ if the length $k-1$ suffix of the sequence for $u$ is the length $k-1$ prefix of the sequence for $v$ \cite{PevznerEuler,Tse}.  
Assuming the debruijn graph is formed using the true $k$-deck of the sequence, paths in the debruijn graph then correspond to possible reconstructions of the sequence.  If we know the string length $n$ as in the trace reconstruction problem, then there is ambiguity in the reconstruction if certain cycle structures exist in the graph (See Figure \ref{figure:fail_example})


\begin{figure} 
	\centering
	\includegraphics[width=0.3\linewidth]{"Ambiguous_kmer_graph.png"}
	\caption{Example of structure in condensed debruijn graph formed from the $k$-deck where there is ambiguity in the reconstruction (a condensed debruijn graph has adjacent nodes combined if they all have one in-edge and one out-edge).  Let $A,B,C,D,E$ represent binary strings that form a condensed debruijn graph.   Both $ABCBDBE$ and $ABDBCBE$ are possible reconstructions given this graph.  However, given the traces, it should be easy to distinguish whether $C$ comes first or $D$ comes first in the source string $s$ if $C$ and $D$ are sufficiently different.
	}
	\label{figure:fail_example}
	\vspace{-3mm}
\end{figure}

A classical result by Ukkonen~\cite{ukkonen} provides a necessary and sufficient condition on the sequence $s$ and $k$ for the $k$-deck to uniquely determine $s$.  This condition involves limiting the length of certain structures of repeated substrings in $s$ to be at most $k-1$.

\iscomment{Avoid saying ``the paper'' so much. Better to say ``Servedio et al. introduced'' (or whoever the first author is)}
The paper that introduced trace reconstruction in the smoothed complexity model \cite{Servedio} uses the simple fact that if there are no repeated substrings of length $k-1$ or greater in the source string $s$, then the $k$-deck uniquely determines $s$.  Recall that the smoothed complexity model requires any string that is passed through a binary symmetric channel before trace generation to be reconstructed with high probability.  The paper then proceeds to prove that for an arbitrary string, the $(\log n)$-deck can be reconstructed with high probability using $\text{poly}(n)$ traces, and prove there won't \iscomment{will not} be any repeats in the source string of length $\geq (\log n-1)$ \iscomment{in text, write ``at least'' instead of $\geq$} with high probability after it is passed through binary symmetric channel, thereby proving that $\text{poly}(n)$ traces suffice for trace reconstruction in the smoothed complexity model.
The paper \cite{Narayanan} provides a similar result on reconstructing the $(100\log n)$-deck for circular strings in $\text{poly}(n)$ time.  

The $k$-deck alone does not give information about the location of $k$-mers in the sequence $s$. However, the set of traces can provide a lot \iscomment{don't use ``a lot'' in formal writing} of information about about these locations.  There are obvious examples where the debruijn \iscomment{de Bruijn} graph formed by the $k$-deck has cycles that do not allow for a unique reconstruction, but the set of traces very clearly reveal the correct reconstruction in conjunction with the correct debruijn graph (see Figure  \ref{figure:fail_example}).
Making use of the information about kmer \iscomment{$k$-mer} location provided in the set of traces, we introduce a novel statistic of the traces that measures the density of a kmer in a given location of $s$.
For a substring $z \in \{0, 1\}^k$, let $\mathcal{I}_{s, z} \in \{0, 1\}^{(n-k+1) \times 1}$ \iscomment{no need for $\times 1$ for vector dimensions} be the vector of indicator random variables such that $\mathcal{I}_{s, z}[j] = \mathbbm{1}\{s_{j:j+k-1} = z \}$. 
Notice that the set of $\mathcal{I}_{s, z}$ for all $z \in \{0, 1\}^k$ uniquely determines $s$.  
Let $h(i,j)$ equal the probability that a binomial random variable with $j-1$ trials and probability parameter $1-p$ is equal to $i-1$.
For a length $k$ string $z$ and source string $s$, the the density measure is given by the vector $K_{s,z} \in \mathbb{R}^{(n-k+1) \times 1}$ where
\al{
K_{s,z}[i] & = \sum_{j=1}^{n-k+1} h(i, j) \mathcal{I}_{s, z}[j] \\ & = \sum_{j=1}^{n-k+1} \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{s_{j:j+k-1} = z \}.
}
%for $i \in \{1,2, ..., n-k+1\}.$
$K_{s, z}$ is a smoothed version of the indicator vector $\mathcal{I}_{s, z}$, and is a measure of density of the string $z$ in $s$, where $i/(1-p)$ is the position in $s$ that contributes most to $K_{s,z}[i]$.
Operationally, $K_{s,z}[i]$ is the probability that the beginning of a true copy of $z$ in $s$ gets shifted to position $i$ in a trace $\tilde{S}$ of $s$.  
We define the {\it $k$-density map} of $s$ as the set of all $K_{s,z}$ for all $z \in \{0, 1\}^k$.

For any $k$, we have that the set of $K_{s,z}$ for all $z \in \{0, 1\}^k$ uniquely determines $s$.  
This can be seen by noticing the invertibility of the upper-triangular matrix that transforms the $2^k (n-k+1) \times 1$ binary vector $\mathcal{I}_s$ that is the concatenation of the $\mathcal{I}_{s, z}$ vectors corresponding to each $z$, to the $2^k (n-k+1) \times 1$ vector $K_s$ that is the concatenation of the $K_{s,z}$ vectors corresponding to each $z$.  While invertible, this matrix is very ill-conditioned, making the transformation from $K_{s}$ to $\mathcal{I}_s$ very sensitive to noise in  $K_{s}$.  Since the set of $K_{s}$ uniquely determines $s$, it also uniquely determines the $k$-deck, and can therefore be seen as a generalization of the $k$-deck that provides information about kmer location.  In fact, 
\al{
\sum_{i=1}^{n-k+1} K_{s,z}[i] & = \sum_{i=1}^{n-k+1} \sum_{j=1}^{n-k+1} h(i, j) \mathcal{I}_{s, z}[j] \\ & = \sum_{i=1}^{n-k+1} \sum_{j=1}^{n-k+1} \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{s_{j:j+k-1} = z \}
\\ & =  \sum_{j=1}^{n-k+1} \sum_{i=1}^{n-k+1} \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{s_{j:j+k-1} = z \}
\\ & =  \sum_{j=1}^{n-k+1} \mathbbm{1}\{s_{j:j+k-1} = z \}
}
which shows that the number of times $z$ appears in $s$ is equal to the sum of the entries in $K_{s, z}$.  The $k$-density map can therefore be seen as a generalization of the $k$-deck that provides information about kmer location.

% This can be seen by noticing the invertibility of the matrix that transforms the $2^k n \times 1$ binary vector that is equal to one at the position corresponding to kmer $z$ and source string position $i$ if and only if $s_i = z$, to the $2^k n \times 1$ vector containing $K_{s,z,i}$ for all $i$ and $z$.  While invertible, this matrix is very ill-conditioned, making the transformation from $K_{s,z,i}$ to $s$ very sensitive to noise in  $K_{s,z,i}$.  Since the set of $K_{s,z,i}$ uniquely determines $s$, it also uniquely determines the $k$-deck, and can therefore be seen as a generalization of the $k$-deck that provides information about kmer location.

In this paper, we show that with high probability,  $K_{s,z,i}$ can be computed  for $z$ of length $c\log(n)$ for constant $c$ with at most $1/f(n)$ error  for any $f(n) \in\text{poly}(n)$ using $\text{poly}(n)$ traces.
There are $2^{c\log n} = n^{c \log 2}$ possible kmers and $n$ possible positions $i$, so the set of all $K_{s,z,i}$ can be computed with at most $1/f(n)$ error for $k=c\log(n)$ using $\text{poly}(n)$ traces.  The proof of this result involves the derivation of several recursions, an application of a known theorem on the combinatorics of strings, and an application of McDiarmid's inequality to prove the estimator is successful with high probability.  This result also yields a useful corollary for distinguishing a broad class of string pairs using $\text{poly}(n)$ traces, adding to the existing literature on the topic \cite{Mcgregor}, \cite{Sudan}, \cite{Bruck}. Using analogous proof techniques, we also improve the upper bound \cite{Servedio2} on the number of traces needed for reconstructing the $k$-deck of $s$ with high probability using $\text{poly}(n)$ traces when $k = c\log n$ for constant $c$, compare this to a lower bound, and give other insights related to the problem.


% In this paper, we introduce a new multi-bit statistic which can be used for distinguishing string pairs, and also for understanding the density of each distinct length $k$ substring at each location in the source string. 
% Using similar proof techniques, we also improve the upper bound on the number of traces needed for reconstructing the multiset of length $k$ substrings of $s$ when $k = c\log n$ for constant $c$, and give other insights related to this problem.  The multiset of length $k$ substrings of $s$ is known as the $k$-deck of $s$, and reconstructing it efficiently is central to trace reconstruction in the smoothed complexity model \cite{Servedio}. 
% The $k$-deck is a common object of interest in sequence reconstruction problems in bioinformatics~\cite{euler,yaakobi,errorcorrection}.
% In particular, a classical result by Ukkonen~\cite{ukkonen} provides necessary and sufficient conditions for when $k$-deck uniquely determines $s$.
%Hence, the $k$-spectrum can be thought of as an intermediate step towards the reconstruction of $s$.

% make sure to cite Narayanan circular trace reconstruction result somewhere

%The challenge with this approach is therefore to find a function that can be estimated accurately enough with as few traces as possible so that a pair of stings can be distinguished with high probability.

%Then, for each pair of strings, the  from the set of traces and check which string it is closer to.
%This methodology was introduced in \cite{Peres} \cite{Servedio}

%In this paper, we focus on efficiently computing statistics about the length $k$ substrings of $s$.  
\section{Notation and Preliminaries}
	
	Strings in this paper are binary and indexed starting from 1. If the index $i$ is negative, $x_i$ is the $(-i)$th element starting from the right end of $x$.  
	Let $s = (s_1, s_1, ..., s_n) \in \{0, 1\}^n$ be the length $n$ string we are trying to recover. $s$ will be called the {\it source string}.
	We denote the {\it channel} that $s$ is passed through by  $\mathcal{C}$.
	In this paper, $\mathcal{C}$ is the {\it deletion channel} $\text{Del}_p$ that deletes each bit of the source string $s$ independently with probability $p$.
	  
	A {\it trace} $\tilde{S}$ of $s$ is defined to be an output of channel  $\mathcal{C}$ when $s$ is passed through it i.e.   $\tilde{S} \leftarrow \mathcal{C}(s)$.  For a string $s$, we denote a trace of $s$ by $\tilde{S}$.
    We define a {\it trace reconstruction algorithm} as an algorithm that reconstructs the source string $s$ given independent traces $\tilde{S}_1, \tilde{S}_2, ..., \tilde{S}_T$ of $s$ with probability at least $1 - \delta$ for some $\delta > 0$.

	
	For a given string $x$, we let $|x|$ denote the length of $x$. For a string $a$ and integer $r$, $a^r$ denotes the string formed by concatenating $r$ copies of $a$.
	A {\it subsequence} of $x$ is a string that can be formed by deleting elements from $x$, and a {\it supersequence} of $x$ is a string that can be formed by inserting elements into $x$. This is in comparison to a {\it substring} of $x$, which is a string that appears in $x$. We let $x[i, j] = (x_i, x_{i+1}, ..., x_j)$ be the substring of $x$ the begins at position $i$ and ends at position $j$. In particular, if $i$ is negative, $x_i$ is the $i$th position starting from the right end of the string. For two stings $x$ and $y$, the number of ways we can make $|y|-|x|$ deletions from $y$ to form $x$ is denoted by $\binom{y}{x}$.  This is a generalization of the binomial coefficient for strings.  Observe that $\binom{y}{x} \leq \binom{|y|}{|x|}$.
	
% 	\begin{Definition} The  {\it length-$k$ substring spectrum} of a string $s$ is defined as the multi-set of all length-$k$ substrings of $s$.  Mathematically, it is defined as
% 	\al{
%     \cS_k(s) = \{ s[i:i+k-1] : i =1,\dots,n-k+1 \}.
%     }
%     We refer to the length-$k$ substring spectrum of $s$ as the {\it $k$-spectrum} of $s$.
%     The {\it support} of the $k$-spectrum of $s$ is the set of all length $k$ substrings of $s$.
%     \end{Definition}
% .
	
% 	\begin{Definition} For a string $x$, the {\it count of $x$ in $s$} is the number of times that $x$ appears as a substring of $s$.  We denote the count of $x$ in $s$ as $N_{x, s}$. We write this as $N_x$ for simplicity when $s$ is clear from context.
% 	\end{Definition}
% 	The values of $N_x$ for all length $k$ strings $x$ that are substrings of $s$ is equivalent to the $k$-spectrum of $s$.    
% 	We let $E_{x, s, p}$ be the expected number of times we see $x$ appear in a trace of $s$ when the deletion probability is $p$.  We write this as $E_x$ when $s$ and $p$ are clear from context.
	
	For a string $x$, let $Y_i(x, s)$ be the set of length $i$ strings such that for each $y \in Y_i(x, s)$, $y$ is a subsequence of $s$, $y$ starts and ends with the same bits as $x$, and $y[2:i-1]$ contains $x[2:k-1]$ as a subsequence. We write this as $Y_i(x)$ when $s$ is clear from context.
	
	
\section{Main results}

% For a length $k$ substring $y$ of $s$, we derive an algorithm for estimating the following quantity 
% \al{
% K_{s,y,i} = \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{s_{j:j+k-1} = y \}.
% }
% $K_{s,y,i}$ is the probability that the beginning of a true copy of $y$ in $s$ gets shifted to position $i$ in a trace $\tilde{S}$ of $s$.  
% $K_{s,y,i}$ acts as a measure of density of the string $y$ in $s$, where $i/(1-p)$ is the position in $s$ that contributes most to $K_{s,y,i}$.
% We prove the following theorem about computing $K_{s,y,i}$ with at most $1/\text{poly}(n)$ error. %$K_{s,y,i}$ runs in polynomial time in $n$ if $k = c \log n$ for constant $c$ if $p < 0.5$.

Let $s \in \{0, 1\}^n $ denote the source string and $z \in \{0, 1\}^{k}$ denote the target string we wish to estimate the density of within $s$.  Let $p$ denote the deletion probability.
\begin{theorem} \label{thm:multibit}
    For $p < 0.5$ and $k = c\log n$ where $c$ is constant, with probability at least $1- \delta$, any entry of $K_{s,z}$ can be estimated with error at most $\epsilon_n$ using $\log(2/\delta) \frac{n}{2 \epsilon_n^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2$ traces where $f(p) = 1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}$. 
    Consequently, with probability at least $1- \delta$,  all entries of all vectors in the $k$-density map can be estimated with error at most $\epsilon_n$ using $\log(2n^{1 + c\log 2}/\delta) \frac{n}{2 \epsilon_n^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2$ traces.
\end{theorem}
% \begin{theorem} \label{thm:multibit}
%     For $p < 0.5$ and $k = c\log n$ where $c$ is constant, with probability at least $1- \epsilon$, any entry of $K_{s,z}$ can be estimated with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$ 
%     Consequently, with probability at least $1- \epsilon$, for all $z$, all entries of $K_{s,z}$ can be estimated with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$ 
% \end{theorem}
In specific, Theorem \ref{thm:multibit} implies that for $p < 0.5$ and $\epsilon_n = 1/g(n)$ where $g(n) = O(\text{poly}(n))$, all entries of all vectors in the $O(\log n)$-density map can be estimated with error at most $\epsilon_n$ using $\text{poly}(n)$ traces.
Theorem \ref{thm:multibit} implies that for two strings $x, y \in \{0,1\}^n$, if there exists some choice of $z$ where $k = c\log n$ and index $i$ such that $|K_{x,z}[i] - K_{y,z}[i]| \geq \text{poly}(n)$, then $x$ can be distinguished from $y$ with high probability using $\text{poly}(n)$ traces.  This is stated formally in Corollary \ref{cor:distinguish_general}.

\begin{cor}
    \label{cor:distinguish_general}
    For $p < 0.5$ and $k = c\log n$ where $c$ is constant, if the strings $x, y \in \{0, 1\}^n$ are such that for some $z \in \{0, 1\}^{c\log n}$ and index $i$, $|K_{x,z}[i] - K_{y,z}[i]| \geq 1/\text{poly}(n)$, then with probability $1-\delta$, $x$ can be distinguished from $y$ using $\text{poly}(n)$ traces.
\end{cor}
Recall that we can recover the $(c\log n)$-deck using $\text{poly}(n)$ traces with high probability as well, however, we can only distinguish between a pair of strings $x,y$ using the $(c\log n)$-deck if $|\Vert K_{x, z}\Vert_1 - \Vert K_{y, z}\Vert_1| \geq 1$ for some $z$ since the number of times $z$ appears in $x$ is equal to $\Vert K_{x, z}\Vert_1$.  
Using Corollary \ref{cor:distinguish_general}, we can distinguish between a pair of strings $x,y$ using $\text{poly}(n)$ traces if $\Vert K_{x, z} - K_{y, z} \Vert_\infty \geq 1/\text{poly}(n)$ for some $z\in \{0 ,1\}^{c\log n}$.  Also observe that due to the equivalence of $\ell_\infty$ norm and $\ell_0$ norm, and the reverse triangle inequality, we have that
\begin{align}
    \Vert K_{x, z} - K_{y, z} \Vert_\infty \geq \frac{1}{n} \Vert K_{x, z} - K_{y, z} \Vert_1 \geq \frac{1}{n} |\Vert K_{x, z}\Vert_1 - \Vert K_{y, z}\Vert_1|.
\end{align}
Thus if $ |\Vert K_{x, z}\Vert_1 - \Vert K_{y, z}\Vert_1| \geq 1/\text{poly}(n)$ for some $z$ where $k = O(\log n)$, then using the $k$-density map, we can distinguish $x$ from $y$ with high probability using $\text{poly}(n)$ traces. This much less restrictive than distinguishing strings using the $k$-deck, further establishing the $k$-density map as a generalization of the $k$-deck.  It is not clear how to find an explicit string pair where the property in Corollary \ref{cor:distinguish_general} does not hold.  

A special case of Corollary \ref{cor:distinguish_general} with a simpler condition is given below.
% \begin{theorem} \label{thm:kdensity}
%     For $p < 0.5$ and $k = c\log n$ where $c$ is constant, the $k$-density map of $s$ can be estimated where each $K_{s,z,i}$ has error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$  
% \end{theorem}
\begin{cor}
    \label{cor:distinguish}
    For $p < 0.5$, if the strings $x, y \in \{0, 1\}^n$ are such that $z \in \{0, 1\}^{k}$ begins at position $i$ in $x$ where $k = O(\log n)$ and, and $z$ does not appear in $y$ at an index in the range $[i - n^{a}, i + n^{a}]$ for some $a > 0.5$, then $x$ can be distinguished from $y$ with high probability using $\text{poly}(n)$ traces.
\end{cor}
Corollaries \ref{cor:distinguish_general} and \ref{cor:distinguish} are an addition to the set of results concerning distinguishing strings, which includes the facts that strings at constant Hamming distance can be distinguished using $\text{poly}(n)$ traces \cite{Mcgregor}, \cite{Sudan}, and strings at constant Levenshtein distance can be distinguished using $\text{poly}(n)$ traces \cite{Bruck}.  Results similar to Corollaries \ref{cor:distinguish_general} and \ref{cor:distinguish} may be able to be obtained from \cite{Chase}.

% Theorem \cite{thm:multibit} can also be used to visualize roughly where in $s$ each length $O(\log n)$ string appears. For each of the $2^{c\log n} = n^{c \log 2}$ possible kmers, we can compute $K_{s,y,i}$ for each of the  $n - k + 1$ possible positions $i$.  
% This yields a plot of the density of $y$ in $s$ for each possible $y$ using $\text{poly}(n)$ traces.   
% In addition, we can use $\text{poly}(n)$ traces to compute the $k$-deck of $s \in \{0,1\}^n$, defined as
% \al{
% \cS_k(s) = \{ s[i:i+k-1] : i =1,\dots,n-k+1 \},
% }
% i.e., the multi-set of all length-$k$ substrings of $s$.  Combining these two statistics, we have an understanding of roughly where copies of $y \in \cS_k(s)$ are located in $s$.
% put figure here

\subsection{$k$-deck reconstruction}

Using our proof technique for estimating $K_{s,y,i}$, we also give a novel proof that the $(c\log n)$-deck where $c$ is constant can be reconstructed using $\text{poly}(n)$ traces for $p < 0.5$ which we discovered independently in 2021, and improve the upper bound \cite{Servedio} on the number of traces for reconstructing the ($c\log n$)-deck of a string for $p < 0.5$ .  

\begin{theorem}
    For deletion probability $p < 0.5$, and any source string $s \in \{0,1\}^n$, we can reconstruct the $(c\log n)$-deck with high probability using
    \al{
     O\left(\log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right)
    }
    traces.
\end{theorem}
The analysis in \cite{Servedio2} proves that 
\al{O\left(n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)}\right)}
traces are sufficient for this task. 
Clearly, the the upper bound we obtain is smaller for $p$ that is not too close to $0$.
% add statement here about how small p needs to be for existing bound to be better.
Using the lower bound we derive below, we see that as $c$ gets close to $0$, our upper bound becomes optimal up to log factors. 
	\begin{theorem}
	    For deletion probability $p$ and any source string $s \in \{0, 1\}^n$, we have that $\Omega(n p (1-p))$ traces are necessary for recovering the $f(n)$-spectrum for any function $f$ such that $f(n) \geq 2$.
	\end{theorem}
	
	\begin{IEEEproof}
	    Suppose we want to decide whether the $k$-deck of the source string is the $k$-deck of $s_1 = 1^{n/2} 0^{n/2}$, or whether it is the $k$-deck of $s_2 = 1^{(n/2) + 1} 0^{(n/2 -1}$.  Observe that for any $k \geq 2$, the only length $n$ string that has the $k$-deck of $s_1$ is $s_1$ itself, and likewise, the only length $n$ string that has the $k$-deck of $s_2$ is $s_2$ itself.  Thus, distinguishing between these two $k$-decks is equivalent to distinguishing between $s_1$ and $s_2$.  From Section 4.2 of \cite{Batu}, we know that $\Omega(n p (1-p))$ traces are necessary for distinguishing between $s_1$ and $s_2$.
	\end{IEEEproof}	    
    We also show that truncating the polynomial in the algorithm from \cite{Servedio} for reconstructing the ($\log n$)-deck  is not necessary to prove that $\text{poly}(n)$ traces suffice for reconstructing the ($\log n$)-deck of a string for $p < 0.5$.

%prove that $\text{poly}(n)$ traces suffice for trace reconstruction in the smoothed complexity model.

% The $k$-deck is a common object of interest in sequence reconstruction problems in bioinformatics~\cite{euler,yaakobi,errorcorrection}.
% In particular, a classical result by Ukkonen~\cite{ukkonen} provides necessary and sufficient conditions for when $\cS_k(s)$ uniquely determines $s$.
% Hence, the $k$-spectrum can be thought of as an intermediate step towards the reconstruction of $s$.  

% 	\subsection{Prior Work}
	
% 	The trace reconstruction problem was first introduced as the sequence reconstruction problem by Levenshtein in 2001 \cite{Lev1}, \cite{Lev2}, where he studied the how many distinct traces of a certain length are necessary in the worst case to reconstruct any source string.  This differs from our setup because the sample complexity required for reconstruction is studied for the worst case set of traces of a given length, i.e. no randomness is used in the generation of the traces.   
    
%     The first study of trace reconstruction where the traces are randomly generated was published in 2004 by Batu, Kannan, Khanna, and McGregor \cite{Batu} where they provided an algorithm that reconstructs a uniformly random source string with high probability using $O(\log(n))$ traces where the deletion probability is $p = O(1/\log(n))$.  The uniformly random source string case was subsequently improved in numerous papers, and currently, the best known algorithm was presented by Holden, Permantle, and Peres.  Their algorithm and uses $\exp(O(\log^{1/3} (n)))$ traces for any deletion probability $p \in [0, 1)$.  Interestingly, their algorithm also handles any constant insertion probability in the range $[0, 1)$.
    
%     The first result on trace reconstruction with random traces for a worst case source string also appeared in \cite{Batu} where they showed that a variation of their algorithm for a random source string reconstructs a worst case source string with high probability using $O(n\log(n))$ traces for deletion probability $p = O(1/n^{1/2 + \epsilon})$.
%     The current best result for reconstructing the worst case source string with constant deletion probability $p \in [0, 1)$ was published in 2021 by Chase where $\exp(\tilde{O}(n^{1/5}))$ traces are used. 
    
    
% \subsection{Our Results}

% \begin{theorem}
%     For $p < 0.5$ and any source string $s \in \{0, 1\}^n$, target string $z \in \{0, 1\}^{k}$ where $k = c\log n$ and $c$ is constant, and index $i$, we can estimate $K_{s,z,i}$ with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$  
% \end{theorem}
% \begin{cor}
%     For $p < 0.5$, if $x \in \{0, 1\}^n$ and $y \in \{0, 1\}^n$ are such that $z \in \{0, 1\}^{k}$ begins at position $i$ in $x$ where $k = O(\log n)$ and, and $z$ does not appear in $y$ at an index in the range $[i - n^{a}, i + n^{a}]$ for some $a > 0.5$, then $x$ can be distinguished from $y$ using $\text{poly}(n)$ traces.
% \end{cor}
% \begin{theorem}
%     For deletion probability $p < 0.5$, and any source string $s \in \{0,1\}^n$, we can reconstruct the $c\log n$-spectrum with high probability using
%     \al{
%      O\left(log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right)
%     }
%     traces.
% \end{theorem}
% The analysis in \cite{Servedio2} proves that 
% \al{O\left(n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)}\right)}
% traces are sufficient for this task.  
% Clearly, the the upper bound we obtain is smaller for $p$ that is not too close to $0$.
% % add statement here about how small p needs to be for existing bound to be better.
% Using the lower bound we derive below, we see that as $c$ gets close to $0$, our upper bound becomes optimal up to log factors. 
% 	\begin{theorem}
% 	    For deletion probability $p$ and any source string $s \in \{0, 1\}^n$, we have that $\Omega(n p (1-p))$ traces are necessary for recovering the $f(n)$-spectrum for any function $f$ such that $f(n) \geq 2$.
% 	\end{theorem}
	
% 	\begin{IEEEproof}
% 	    Suppose we want to decide whether the $k$-spectrum of the source string is the $k$-spectrum of $s_1 = 1^{n/2} 0^{n/2}$, or whether it is the $k$-spectrum of $s_2 = 1^{(n/2) + 1} 0^{(n/2 -1}$.  Observe that for any $k \geq 2$, the only length $n$ string that has the $k$-spectrum of $s_1$ is $s_1$ itself, and likewise, the only length $n$ string that has the $k$-spectrum of $s_2$ is $s_2$ itself.  Thus, distinguishing between these two $k$-spectrums is equivalent to distinguishing between $s_1$ and $s_2$.  From Section 4.2 of \cite{Batu}, we know that $\Omega(n p (1-p))$ traces are necessary for distinguishing between $s_1$ and $s_2$.
% 	\end{IEEEproof}	    

% 	%Unfortunately, the pair of strings used in  \cite{Chase2} for the best known lower bound for worst case trace reconstruction have the same $k$-spectrum for many interesting values of $k$.  


	
\section{Proof of Theorem \ref{thm:multibit}}

For strings $x, y$, let $\binom{y}{x}' = \binom{y[2:-2]}{x[2:-2]}$.  For source string $s$ and length $k$ string $x$, let $E_{s, x, i} = E[\mathbbm{1}\{\tilde{S}[i:i+|z|-1] = z \}]$, and recall that
\al{
K_{s,x}[i] = \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{\tilde{S}[j:j+\ell-1] = x \}.
}
The first part of the proof is a derivation of the following formula
\al{
    K_{s, x, i} = \frac{1}{(1-p)^k}\left( E_{x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_{y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right).
}
This formula for $K_{s, x, i}$ depends only on $E_{s, y, i}$ for all strings $y$, so $K_{s, x, i}$ can be estimated from the easily computable estimates of $E_{s, y, i}$.  Our estimator for $K_{s, x, i}$ is given by
\al{
    \hat{K}_{s, x, i} = \frac{1}{(1-p)^k}\left( \hat{E}_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_{s, y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right)
}
where $\hat{E}_{s, x, i} = \frac{1}{T} \sum_{t = 1}^T \mathbbm{1}\{\tilde{S}_t[i:i+|x|-1] = x \}$.
We then use McDiarmid's inequality to understand how many traces are needed for this estimator of $K_{s, x, i}$ to perform at a certain level of accuracy with high probability.  

To derive our formula for $\hat{K}_{s, x, i}$, we begin by deriving a recursive estimator for $\hat{K}_{s, x, i}$.  We have
\al{
    E_{s, x, i} & = \sum_{\ell = k}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{\tilde{s}_{j:j+\ell-1} = y \}
    \\ & = \sum_{\ell = k}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k K_{s, y, i}.
}
This can be rewritten as the recursive formula
\al{
    K_{s, x, i} & = \frac{1}{(1-p)^k} 
    \left( E_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k K_{s, y, i} \right)
    \\ & = \frac{1}{(1-p)^k} 
    \left( E_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_\ell(x)} (1-p)^\ell \binom{y}{x}'  K_{s, y, i} \left(\frac{p}{1-p}\right)^{\ell - k} \right).
}
This recursive formula can be expanded so that $K_{s, x, i}$ is written only in terms of $E_{s, x, i}$.  
This yields a formula of the form
\begin{align}
	K_{s, x, i} = \frac{1}{(1-p)^k} \left(E_{s, x, i} - \sum_{\ell=k+1}^n \sum_{y \in Y_\ell(x)} E_{s, y, i} a_{y, x, s} \left(\frac{ p}{1-p}\right)^{\ell-k} \right)
\end{align}
where $a_{y, x, s} \in \mathbb{Z}$ is a constant that depends on $y, x, s$.
Observe that $a_{y, x, s}$ obeys the following recursion:  for $y \in Y_\ell(x)$, we have that 
\begin{align}
	a_{y,x,s} = \binom{y[2:-2]}{x[2:-2]} - \sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x)} a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}. 
\end{align}
This is because as we expand the recursive formula for $K_{s, x, i}$ one step at a time, we observe that every time we obtain a new term involving $E_{s, y, i}$ in the expansion with coefficient $c_y \left(\frac{p}{1-p}\right)^{|y| - k}$, at the next step of the expansion we obtain a term involving $E_{s, z, i}$ with coefficient $-c_y \binom{z[2:-2]}{y[2:-2} \left(\frac{p}{1-p}\right)^{|z| - k}$ for every $z \in \cup_{\ell = |y| + 1}^n Y_\ell(y)$.

We proceed to prove that for any $x$, $y$, $s$, we then have that 
\begin{align}
	a_{y,x,s} = (-1)^{|y| -|x|+1} \binom{y[2:-2]}{x[2:-2]}.
\end{align}
If $|y| - |x| = 1$, this clearly holds.  
Suppose it holds for $|y| - |x| <  m$.  Then if $|y| - |x| =  m$, we have that
\begin{align}
	a_{y,x,s} & = \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}
	\\ & =  \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| -|x| + 1} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
	\\ & =  \binom{y[2:-2]}{x[2:-2]} + 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| + |x|} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
	\\ & = \binom{y[2:-2]}{x[2:-2]} + \left(- \binom{y[2:-2]}{x[2:-2]} - (-1)^{|y| + |x|} \binom{y[2:-2]}{x[2:-2]}\right)
	\\ & =  (-1)^{|y| - |x| + 1} \binom{y[2:-2]}{x[2:-2]}.
\end{align}	
where the fourth line follows from Corollary (6.3.9) in \cite{Lothaire}, 
which states that 
for some alphabet $\Sigma$ and all strings $f, g$ we have
\begin{align}
    \sum_{h} (-1)^{|g| + |h|} \binom{f}{h} \binom{h}{g} = \delta_{f, g}
\end{align}
where $\delta_{f, g} = 0$ if $f \neq g$, and $\delta_{f, g} = 1$ if $f = g$.
Therefore, we can write $K_{s, x, i}$ only in terms of the terms $E_{s, y, i}$ for all $y$:
\al{
    K_{s, x, i} = \frac{1}{(1-p)^k}\left( E_{x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_{y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right).
}

\subsection{sample complexity analysis}
Changing a single bit in the $t$th trace $\tilde{S}_t$ changes the estimator by at most
\begin{align}
    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + \sum_{\ell = k+1}^n 2 \max_{y \in Y_\ell (x)} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left(1 + \sum_{\ell = k+1}^n 2  \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right).
\end{align}
%For $k = c\log(n)$ for constant $c$ and $p < 0.5$, 
To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
\begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( 1 + 2 n \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{\ell-c\log(n)}\right)
\\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( 1 + 2 n \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell-c\log(n)}\right)
\\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{1 + c \log(\frac{1-p}{p})}  \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell}\right).
\end{align}
where we take $\log()$ to have base 2. 
We have that
\begin{align}
    & \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell}
    \\ & \leq \max_{\ell \in [c\log(n)+1, n]} 2^{\ell H(c\log(n)/\ell)} \left(\frac{p}{1-p}\right)^{\ell}
    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
\end{align}
because the maximizing $\ell$ is given by $\ell^* = \frac{\log(n^c)}{1- p/(1-p)}$ .
This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
\begin{align}
    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
\end{align}
where $q = p/(1-p)$,
the function is a differentiable for $x \in (c\log(n)+1, n),$
and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
\begin{align}
    - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
\end{align}
which is negative.
We therefore have that we  have that 
\begin{align} 
    b &
    \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{1 + c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
\end{align}    
when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
Let
\begin{align}
    f(p) = 1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
\end{align}
Plugging this into McDiarmid's inequality,  we have
\begin{align}
	\Pr \left(|\hat{K}_{s,x,i} - K_{s,x,i}| \geq \epsilon \right) & \leq 2\exp \left(-\frac{2\epsilon^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{f(p)}  \right) \right)^2}\right)
	\\ & = 2\exp \left(-\frac{2T\epsilon^2}{n \left(\frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{f(p)}  \right)\right)^2}\right)
\end{align}
Setting $\delta = \Pr \left(|\hat{K}_{s,x,i} - K_{s,x,i}| \geq \epsilon \right)$, we have
\begin{align}
    T = \log(2/\delta) \frac{n}{2\epsilon^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2
\end{align}
traces suffices for recovering $K_{s,x,i}$ with error $< \epsilon$ with probability at least $1 - \delta$.

% \subsection{analysis for $k = c\sqrt{n}$}

% Using McDiarmid's inequality as before, we have that changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
% \begin{align}
%     b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + \sum_{\ell = k+1}^n 2 \max_{y \in Y_\ell (x)} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left(1 + \sum_{\ell = k+1}^n 2  \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell}{k} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   2^{\ell H(k/\ell)} \left(\frac{p}{1-p}\right)^{\ell-k}\right).
% \end{align}
% For $k = c\sqrt{n}$, we have 
% \al{
%     \frac{d}{d\ell} 2^{\ell H(k/\ell)} \left(\frac{p}{1-p}\right)^{\ell-k} = \left(\frac{p}{1-p}\right)^{\ell - \sqrt{n}} \left(1 - \frac{\sqrt{n}}{\ell}\right)^{\sqrt{n} - \ell} \left(\frac{\sqrt{n}}{\ell}\right)^{-\sqrt{n}} \left(\log(\frac{p}{1-p}) -  \log(1 - \frac{\sqrt{n}}{\ell})\right)
% }
% Let $q = \frac{p}{1-p}$. Setting the derivative equal to zero and solving for $\ell$, we obtain 
% \al{
%     \ell^* = \frac{\sqrt{n}}{1 - q}.
% }
% Plugging this in, we obtain
% \al{
%     q^{\sqrt{n}\frac{q}{1 - q}} 2^{\frac{\sqrt{n} ((q - 1) \log(1 - q) - q \log(1 - \sqrt{n} (1 - q)))}{(1 - q) \log(2)}}.
% }

	\section{$K$-deck Reconstruction}
	
	In order to recover the $k$-spectrum for source string $s$ and deletion probability $p$, we need to estimate $N_x$ for each of the possible $2^k$ strings of length $k$.  However, it is not immediately clear how to construct an estimator $\hat{N}_x$. Our approach is to first write $N_x$ in terms of $E_y$ for all strings $y \in \cup_{i = k+1}^n Y_i(x)$.  $E_y$ is easily estimated as $\hat{E}_y = \frac{1}{T}\sum_{i = 1}^T (\text{\# of times $y$ appears as a substring in trace $t_i$})$, which we subsequently plug into the formula we derive for $N_x$ in order to form our estimate $\hat{N}_x$.

    Our estimator is given by
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	\end{align}
	which we then round to the nearest integer.  Observe that if the error in the estimate of $N_x$ is $< 1/2$, then we will estimate $N_x$ correctly after rounding.
	
	For any $k$, our estimator can be computed in $O(T n^2 \binom{n}{k})$ time because for each of the $T$ traces, we need to compute $\binom{y[2:-2]}{x[2:k-1]}$ for each of the $O(n^2)$ substrings in the trace, and computing $\binom{y[2:-2]}{x[2:k-1]}$ using a brute force approach takes $O(\binom{n}{k})$ time.

    In order to derive our estimator, we begin by writing a recursive formula for $N_x$ which we subsequently use to obtain a nonrecursive formula for $N_x$ in terms of $E_y$s.  This nonrecurive formula yeilds our estimator.
	

	
	\begin{theorem} \label{theorem:rec_estimator}
	    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
		\begin{align}
			N_x = \frac{1}{(1-p)^k}\left(E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} (1-p)^i N_{y} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
		\end{align}  
	\end{theorem}	
	
	\begin{IEEEproof}
		In this proof, let $E_{\hat{z}} = (1-p)^{|z|} N_z$ i.e. $E_{\hat{z}}$ is the expected number of times a copy of $z$ (contained as a substring of $s$) is unaffected by deletions in a trace.  $E_{\hat{z}} = 0$ if and only if $z$ is not a substring of $s$.   Observe that $E_{\hat{x}}$ is equal to $E_x$ minus the expected number of copies of $x$ that appear in the trace due to deletions.  This follows from linearity of expectation applied to the indicator random variables that copies of $x$ are formed using bits at specific positions in $s$ as the start and end bits of the copies of $x$.
		Any copy of $x$ in a trace that is formed from deletions is created by  deleting elements at internal positions in some $y \in Y_i(x)$ for some $i > k$ that is a true copy of $y$ in $s$.
		For a  particular $i \in \mathbb{N}$, we have that for a position $r$ in $s$ such that $ s[r:r+i-1] = y \in 
		Y_i(x)$, the expected value of the indicator random variable that a copy of $x$ is formed using the start and end bits of $s[r:r+i-1]$ is given by $(1-p)^i \binom{y[2:i-1]}{x[2:k-1]}\frac{ p^{i - k}}{(1-p)^{i-k}}$.  If there are $c$ such positions $r$ for this $y$, we have that the expected number of times $x$ arises using these pairs of bits as the start and end bits in the copy of $x$ is given by   
		\begin{align}
			E_{\hat{y} \to x} = c \binom{y[2:-2]}{x[2:-2]} (1-p)^k p^{i - k} = c (1-p)^i \binom{y[2:-2]}{x[2:-2]} \frac{ p^{i - k}}{(1-p)^{i-k}} = E_{\hat{y}} \binom{y[2:-2]}{x[2:-2]} \frac{ p^{i - k}}{(1-p)^{i-k}}
		\end{align} by applying linearity of expectation to the sum of the indicator random variables for the terms corresponding to each copy of $y$ in $s$.   
		Then summing over all $y \in Y_i(x)$ for all valid $i$, we are left with  
		\begin{align}
			\sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{\hat{y}} \binom{y[2:i-1]}{x[2:k-1]} \frac{ p^{i - k}}{(1-p)^{i-k}}.
		\end{align}  
		by linearity of expectation.
		Thus, we have
		\begin{align}
			E_{\hat{x}} = E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{\hat{y}} \binom{y[2:i-1]}{x[2:k-1]} \frac{ p^{i - k}}{(1-p)^{i-k}}.
		\end{align} 
		%For the largest value of $i$ such that $Y_i(x) \neq \emptyset$, There is clearly only one element in $Y_i(x)$, and there is no way to form this $y$ from deletions so $E_{\hat{y}} = E_{y}$.
	\end{IEEEproof}

	
	\begin{theorem} \label{theorem:estimator}
	    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
	    \begin{align}
	        N_x = \frac{1}{(1-p)^k}\left( E_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	    \end{align}
	\end{theorem}	
	
	\begin{IEEEproof}
	    We can expand the recursion in Theorem \ref{theorem:rec_estimator} so that $N_x$ is only written in terms of $E_y$s. 
	    The resulting formula will be of the following form
    	\begin{align}
    		N_{x} = \frac{1}{(1-p)^k} \left(E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{y} a_{y, x, s} \left(\frac{ p}{1-p}\right)^{i-k} \right)
    	\end{align}
    	where $a_{y, x, s} \in \mathbb{Z}$ is a constant that depends on $y, x, s$.
    	We observe that $a_{y, x, s}$ obeys the following recursion:  for $y \in Y_i(x)$, we have that 
    	\begin{align}
    		a_{y,x,s} = \binom{y[2:-2]}{x[2:-2]} - \sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x)} a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}. 
    	\end{align}
    	This is because as we expand the recursive formula for $N_x$ one step at a time, we observe that every time we obtain a new term involving $E_y$ in the expansion with coefficient $c_y \left(\frac{p}{1-p}\right)^{|y| - k}$, at the next step of the expansion we obtain a term involving $E_z$ with coefficient $-c_y \binom{z[2:-2]}{y[2:-2} \left(\frac{p}{1-p}\right)^{|z| - k}$ for every $z \in \cup_{i = |y| + 1}^n Y_i(y)$.
    	
    	We proceed to prove that for any $x$, $y$, $s$, we then have that 
		\begin{align}
			a_{y,x,s} = (-1)^{|y| -|x|+1} \binom{y[2:-2]}{x[2:-2]}.
		\end{align}
		If $|y| - |x| = 1$, this clearly holds.  
		Suppose it holds for $|y| - |x| <  m$.  Then if $|y| - |x| =  m$, we have that
		\begin{align}
			a_{y,x,s} & = \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}
			\\ & =  \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| -|x| + 1} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
			\\ & =  \binom{y[2:-2]}{x[2:-2]} + 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| + |x|} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
			\\ & = \binom{y[2:-2]}{x[2:-2]} + \left(- \binom{y[2:-2]}{x[2:-2]} - (-1)^{|y| + |x|} \binom{y[2:-2]}{x[2:-2]}\right)
			\\ & =  (-1)^{|y| - |x| + 1} \binom{y[2:-2]}{x[2:-2]}.
		\end{align}	
		where the fourth line follows from Corollary (6.3.9) in \cite{Lothaire}, 
		which states that 
		for some alphabet $\Sigma$ and all strings $f, g$ we have
		\begin{align}
		    \sum_{h} (-1)^{|g| + |h|} \binom{f}{h} \binom{h}{g} = \delta_{f, g}
		\end{align}
		where $\delta_{f, g} = 0$ if $f \neq g$, and $\delta_{f, g} = 1$ if $f = g$.
	\end{IEEEproof}

    \section{Analysis of Estimator (Improved and Simplified)}
	McDiarmid's inequality states the following.  Let $X_1, ..., X_m$ are iid random variables. Suppose the function $f$ has the property that for any sets of values $x_1, x_2, ..., x_m$ and $x'_1, x'_2, ..., x'_m$ that only differ at the $i$th random variable, it follows that 
	\begin{align}
		&
		|f(x_1, x_2, ..., x_m) - f(x'_1, x'_2, ..., x'_m)| \leq b_i.
	\end{align} 
	Then, for any $t > 0$, we have that 
	\begin{align}
		\Pr(f(X_1, X_2, ..., X_m) - \mathbb{E}[f(X_1, X_2, ..., X_m)] \geq t) \leq \exp \left(-\frac{2t^2}{\sum_{i = 1}^m b_i^2}\right). 
	\end{align}
	Applying this to our problem, we set $f = \hat{N}_x$ and we take each random variable $X_i$ to be an indicator of whether a particular bit in $s$ is deleted in a particular trace.  
	
    Recall that our estimator is given by 
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	\end{align}
	Changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
	\begin{align}
	    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( \min(k, n-k+1) + \sum_{i = k+1}^n 2 \min(i, n-i+1) \max_{y \in Y_i (x)} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + \sum_{i = k+1}^n 2 i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 n \max_{i \in [k+1, n]} i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 n^2 \max_{i \in [k+1, n]}  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	\end{align}
	To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
    \begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 n^2 \max_{i \in [c\log(n)+1, n]}  \binom{i-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 n^2 \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log(\frac{1-p}{p})}  \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}\right).
	\end{align}
	where we take $\log()$ to have base 2. 
	We have that
	\begin{align}
	    & \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq \max_{i \in [c\log(n)+1, n]} 2^{i H(c\log(n)/i)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
	    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
	\end{align}
	The maximizer is given by $i = \frac{\log(n^c)}{1- p/(1-p)}$ .
	This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
	\begin{align}
	    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
	\end{align}
	where $q = p/(1-p)$,
	the function is a differentiable for $x \in (c\log(n)+1, n),$
	and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
	\begin{align}
        - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
	\end{align}
    which is negative.
    We therefore have that 
        \begin{align} b &
        \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
        \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
	\end{align}    
    when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
    Let
    \begin{align}
        f(p) = 2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
    \end{align}
	Plugging this into McDiarmid's inequality, and setting $\epsilon = 1/2$,  we have
	\begin{align}
		\Pr \left(\hat{N}_x - N_x \geq \frac{1}{2} \right) & \leq \exp \left(-\frac{2\left( \frac{1}{2}\right)^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right) \right)^2}\right)
		\\ & = \exp \left(-\frac{T}{2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2}\right)
    \end{align}
    Setting $\delta = \Pr \left(\hat{N}_x - N_x \geq \frac{1}{2} \right)$, we have
    \begin{align}
        T = \log(1/\delta) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2
    \end{align}
    traces suffices for recovering $N_x$ with probability at least $1 - \delta$.

	There are $2^{c\log(n)}$ strings $x$ in total to test, so if we want to upper bound the probability of making making a mistake in estimating any $x$ using the number of traces above, we can use the union bound. Setting $\delta = \frac{1}{n2^{c\log(n)}}$, we have
    \begin{align}	
        T & \sim \log(n2^{c\log(n)})2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = \log(e^{log(n)+ c\log(n) \log(2)}) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = 2n (log(n)+ c\log(n) \log(2))  \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = O(\text{poly}(n)).
    \end{align}	
    traces suffice. 
    
    Using the union bound on the probability of error over all $2^{c\log(n)}$ kmers, we get a probability of error upper bounded by
	\begin{align}
		2^{c\log(n)} \frac{1}{n2^{c\log(n)}} = \frac{1}{n}.
	\end{align}
	Thus for $p \in [0, .5)$, we reconstruct the  the $c\log(n)$-spectrum of $s$ with probability greater than $1 - \frac{1}{n}$ using $O(\text{poly}(n))$ traces.  	


\section{Comparison with results from Servedio paper}

\subsection{Difference in Techniques}
Recall that our main structural result is the following theorem.
\begin{theorem} 
    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
    \begin{align}
        N_x = \frac{1}{(1-p)^k}\left( E_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
    \end{align}
\end{theorem}	
To estimate $N_x$ for $p < 0.5$, we  directly estimate $ E_y$ from the traces and calculate $\binom{y[2:i-1]}{x[2:k-1]}$ for $y \in Y_i(x), \;  i \geq k$.
In the Servedio paper, they first present an algorithm for $p < 0.5$ where they instead estimate $E[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, y)]$ from the traces and estimate $N_x$ using the formula 
\al{
    N_x = \frac{1}{(1-p)^k} \sum_{\substack{\alpha \in \mathbb{Z}_{\geq 0}^{k-1} \\ |\alpha| \leq n-k}} E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right] \left(\frac{-p}{1-p}\right)^{|\alpha|}
}
where $*$ is the wildcard symbol and $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)$ is the number of times a substring of the form $x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}$ appears in a trace $t$ of $s$ with deletion probability $p$, and $|\alpha| = \sum_{i=1}^{k-1} |\alpha_i|$ for $\alpha \in \mathbb{Z}_{\geq 0}^{k-1}$.
Observe that we derived the same polynomial as the Servedio paper but in a different form.  Our proof is very different from theirs in that we first derive a recursive estimator of $N_x$ and then use structural knowledge of $\binom{y[2:i-1]}{x[2:k-1]}$ to prove its equivalence to the polynomial above.

In their initial algorithm for $p < 0.5$, they just bound the error of the estimate of each $ E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right]$ using a Chernoff bound and the fact that $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t) \in [0, n]$.  For this reason, their initial algorithm for calculating $N_x$ where $|x| = k$ for $p < 0.5$ uses $n^{O(k)} \cdot \log(1/\delta)$ traces and running time.  For $k = c \log(n)$ which is what both their paper and our paper are interested in, their number of traces and running time is superpolynomial  in $n$ whereas ours is polynomial in $n$.  

In their improved algorithm for $p < 0.5$ that uses polynomial runtime and number of traces in $n$, they estimate $N_x$ using only estimates of $E_y$ for substrings $y$ of length at most $d + k$ where $d := \frac{e^2}{1/2 - \delta} \left( k\log \left(\frac{e^2}{1/2 - \delta}\right) + \log(n) \right)$.  The formula they use is then
\al{
    N_x = \frac{1}{(1-p)^k} \sum_{\substack{\alpha \in \mathbb{Z}_{\geq 0}^{k-1} \\ |\alpha| \leq d}} E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right] \left(\frac{-p}{1-p}\right)^{|\alpha|}.
}
They then prove that the sum of the terms in the polynomial for strings $y$ of length $>d+k$ are small and they again bound the error of the estimate of each $ E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right]$ using a Chernoff bound and the fact that $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t) \in [0, n]$. 

This is different from our analysis because we don't truncate the polynomial, and we use McDiamids inequality to bound the error in the entire polynomial instead of using a Chernoff bound to  bound to the error of the estimate of each coefficient in the polynomial followed by a union bound.  


\subsection{Comparison of Results}

In the Serverdio paper, the number of traces used by their algorithm to recover $N_x$ with probability at least $1- \delta$ for $p < 1/2$ is
\begin{align}
    O((M^2 2^k)^2) \log\left(\frac{M}{\delta}\right) & = O\left( \left( \left(n \left(\frac{e^2}{1/2 - p}\right)^{3k} \right)^2 2^k\right)^2\right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3k}}{\delta}\right)
    \\ & = O\left( n^4  \left(\frac{e^2}{1/2 - p}\right)^{12k}  4^k \right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3k}}{\delta}\right).
\end{align}
For $k = c \log(n)$, we have that the number of traces used is
\begin{align}
    & O\left( n^4  \left(\frac{e^2}{1/2 - p}\right)^{12c\log(n)}  4^{c\log(n)} \right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3c\log(n)}}{\delta}\right)
    \\ & = O\left( n^4  n^{12c \left(\frac{e^2}{1/2 - p}\right)}   n^{c\log(4)} \right) \log\left(\frac{n \cdot n^{3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right)
    \\ & = O\left( n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)} \right) \log\left(\frac{n^{1 + 3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right)
    \\ & = O\left( n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)} \right) \log\left(\frac{n^{1 + 3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right).
\end{align}
In comparison, the number of traces used by our algorithm for recovering $N_x$ with probability at least $1- \delta$ for $p < 1/2$ is
\begin{align}
    & \log(1/\delta) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2
    \\ & = O \left(n^{1 + 2 \left(f(p) + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
\end{align}
traces where
\begin{align}
    f(p) & = 2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}.
\end{align}
Observe that we can upper bound $f(p)$ as follows
\begin{align}
    f(p)  \leq 2 + c \log((1-p)/p) + \frac{c }{1- p/(1-p)}
\end{align}
by using the fact that $H(x) \leq 1$ for all $x$ and $\log(p/(1-p)) < 0$ for $p < 0.5$. 
Thus, the number of traces needed by our algorithm is upper bounded by 
\begin{align}
    & O \left(n^{1 + 2 \left(2 + c \log((1-p)/p) + \frac{c }{1- p/(1-p)} + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
    \\ & = O\left(n^{5 + 2 c \log((1-p)/p) + \frac{2c }{1- p/(1-p)} + 2c\log\left(\frac{1}{1-p}\right)}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c (\log(1/p) + \frac{1 }{1- p/(1-p)})}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c (\log(1/p) + \frac{1-p}{1-2p})}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)\log(1/\delta).
\end{align}
Recall that the exponent of $n$ in the number of traces used by Servedio's algorithm is 
\al{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4).}
Clearly, the number of traces used by our algorithm is smaller for $p$ close to $0.5$ and $c=1$ which is the $c$ they used in their paper.

\section{Analysis of Truncated Estimator}
	McDiarmid's inequality states the following.  Let $X_1, ..., X_m$ are iid random variables. Suppose the function $f$ has the property that for any sets of values $x_1, x_2, ..., x_m$ and $x'_1, x'_2, ..., x'_m$ that only differ at the $i$th random variable, it follows that 
	\begin{align}
		&
		|f(x_1, x_2, ..., x_m) - f(x'_1, x'_2, ..., x'_m)| \leq b_i.
	\end{align} 
	Then, for any $t > 0$, we have that 
	\begin{align}
		\Pr(f(X_1, X_2, ..., X_m) - \mathbb{E}[f(X_1, X_2, ..., X_m)] \geq t) \leq \exp \left(-\frac{2t^2}{\sum_{i = 1}^m b_i^2}\right). 
	\end{align}
	Applying this to our problem, we set $f = \hat{N}_x$ and we take each random variable $X_i$ to be an indicator of whether a particular bit in $s$ is deleted in a particular trace.  
	
    Recall that the truncated estimator from the Servedio paper written in our form is given by 
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^d \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right)
	\end{align}
	where 
	\begin{align}
	    d = \frac{e^2}{1/2 - p} \left( k \ln \frac{e^2}{1/2 - p} + \ln n \right).
	\end{align}
	Changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
	\begin{align}
	    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( \min(k, n-k+1) + \sum_{i = k+1}^d 2 \min(i, n-i+1) \max_{y \in Y_i (x)} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + \sum_{i = k+1}^d 2 i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 d \max_{i \in [k+1, d]} i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 d^2 \max_{i \in [k+1, d]}  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	\end{align}
	To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
    \begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 d^2 \max_{i \in [c\log(n)+1, d]}  \binom{i-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 d^2 \max_{i \in [c\log(n)+1, d]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2d^2 n^{c \log(\frac{1-p}{p})}  \max_{i \in [c\log(n)+1, d]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}\right).
	\end{align}
	where we take $\log()$ to have base 2. 
	We have that
	\begin{align}
	    & \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq \max_{i \in [c\log(n)+1, n]} 2^{i H(c\log(n)/i)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
	    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
	\end{align}
	The maximizer is given by $i = \frac{\log(n^c)}{1- p/(1-p)}$ .
	This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
	\begin{align}
	    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
	\end{align}
	where $q = p/(1-p)$,
	the function is a differentiable for $x \in (c\log(n)+1, n),$
	and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
	\begin{align}
        - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
	\end{align}
    which is negative.
    We therefore have that 
        \begin{align} b &
        \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
        \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
	\end{align}    
    when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
    Let
    \begin{align}
        f(p) = c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
    \end{align}
	Plugging this into McDiarmid's inequality, and setting $\epsilon = 1/5$,  we have
	\begin{align}
		\Pr \left(\hat{N}_x - N_x \geq \frac{1}{5} \right) & \leq \exp \left(-\frac{2\left( \frac{1}{5}\right)^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right) \right)^2}\right)
		\\ & = \exp \left(-\frac{T}{\frac{25}{2}n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2}\right)
    \end{align}
    Setting $\delta = \Pr \left(\hat{N}_x - N_x \geq \frac{1}{5} \right)$, we have
    \begin{align}
        T = \log(1/\delta) \frac{25}{2} n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2
    \end{align}
    traces suffices for recovering $N_x$ with probability at least $1 - \delta$.

\subsection{comparison}

The number of traces needed to recover $N_x$ with probability at least $1- \delta$ for $p < 1/2$ using the truncated estimator is
\begin{align}
    & \log(1/\delta) \frac{25}{2} n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2
    \\ & = O \left(d^4 n^{1 + 2 \left(f(p) + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
\end{align}
traces where
\begin{align}
    f(p) & = c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}.
\end{align}
Observe that we can upper bound $f(p)$ as follows
\begin{align}
    f(p)  \leq c \log((1-p)/p) + \frac{c }{1- p/(1-p)}
\end{align}
by using the fact that $H(x) \leq 1$ for all $x$ and $\log(p/(1-p)) < 0$ for $p < 0.5$. 
Thus, the number of traces needed by our algorithm is upper bounded by 
\begin{align}
    & O \left(d^4 n^{1 + 2 \left(c \log((1-p)/p) + \frac{c }{1- p/(1-p)} + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
    \\ & = O\left(d^4 n^{1 + 2 c \log((1-p)/p) + \frac{2c }{1- p/(1-p)} + 2c\log\left(\frac{1}{1-p}\right)}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c (\log(1/p) + \frac{1 }{1- p/(1-p)})}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c (\log(1/p) + \frac{1-p}{1-2p})}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)\log(1/\delta)
    \\ & = 	 O\left(log^4(n) \cdot n^{1 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)
    \\ & = 	 O\left(log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right).
\end{align}
Recall that the exponent of $n$ in the number of traces used by Servedio's algorithm is 
\al{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4).}
Clearly, the number of traces used by our algorithm is smaller for $p$ close to $0.5$ and $c=1$ which is the $c$ they used in their paper.



==> notation.tex <==



	
	Strings in this paper are binary and indexed starting from 1. If the index $i$ is negative, $x_i$ is the $(-i)$th element starting from the right end of $x$.  
	\iscomment{weird to have the indices starting from 1 and the negative indices notation. What is $x_0$? Do we need negative indices?}
	Let $s = (s_1, \dots, s_n) \in \{0, 1\}^n$ be the length-$n$ string we are trying to recover. The string $s$ will be called the source string.
	\iscomment{Seems unnecessary to define a random channel $\cC$ and a channel $\text{Del}_p$, since there is only one channel in the paper. Just directly describe how the traces are generated}
	We denote the {\it channel} that $s$ is passed through by  $\mathcal{C}$.
	In this paper, $\mathcal{C}$ is the {\it deletion channel} $\text{Del}_p$ that deletes each bit of the source string $s$ independently with probability $p$.
	  
	A trace $\tilde{S}$ of $s$ is defined to be an output of channel  $\mathcal{C}$ when $s$ is passed through it i.e.   $\tilde{S} \leftarrow \mathcal{C}(s)$.  For a string $s$, we denote a trace of $s$ by $\tilde{S}$.
    We define a {\it trace reconstruction algorithm} as an algorithm that reconstructs the source string $s$ given independent traces $\tilde{S}_1, \tilde{S}_2, \dots, \tilde{S}_T$ of $s$ with probability at least $1 - \delta$ for some $\delta > 0$.

	
	For a given string $x$, we let $|x|$ denote the length of $x$. For a string $a$ and integer $r$, $a^r$ denotes the string formed by concatenating $r$ copies of $a$.
	A {\it subsequence} of $x$ is a string that can be formed by deleting elements from $x$, and a {\it supersequence} of $x$ is a string that can be formed by inserting elements into $x$. This is in contrast to a {\it substring} of $x$, which is a string that appears in $x$. We let $x[i, j] = (x_i, x_{i+1}, \dots, x_j)$ be the substring of $x$ the begins at position $i$ and ends at position $j$. In particular, if $i$ is negative, $x_i$ is the $i$th position starting from the right end of the string. For two stings $x$ and $y$, the number of ways we can make $|y|-|x|$ deletions on $y$ to form $x$ is denoted by $\binom{y}{x}$.
	This is a generalization of the binomial coefficient for strings. Observe that $\binom{y}{x} \leq \binom{|y|}{|x|}$.
	
% 	\begin{Definition} The  {\it length-$k$ substring spectrum} of a string $s$ is defined as the multi-set of all length-$k$ substrings of $s$.  Mathematically, it is defined as
% 	\al{
%     \cS_k(s) = \{ s[i:i+k-1] : i =1,\dots,n-k+1 \}.
%     }
%     We refer to the length-$k$ substring spectrum of $s$ as the {\it $k$-spectrum} of $s$.
%     The {\it support} of the $k$-spectrum of $s$ is the set of all length $k$ substrings of $s$.
%     \end{Definition}
% .
	
% 	\begin{Definition} For a string $x$, the {\it count of $x$ in $s$} is the number of times that $x$ appears as a substring of $s$.  We denote the count of $x$ in $s$ as $N_{x, s}$. We write this as $N_x$ for simplicity when $s$ is clear from context.
% 	\end{Definition}
% 	The values of $N_x$ for all length $k$ strings $x$ that are substrings of $s$ is equivalent to the $k$-spectrum of $s$.    
% 	We let $E_{x, s, p}$ be the expected number of times we see $x$ appear in a trace of $s$ when the deletion probability is $p$.  We write this as $E_x$ when $s$ and $p$ are clear from context.
	
	\iscomment{Maybe $Y_i$ should only be defined when it's needed? It feels very specific here}
	
	For a string $x$, let $Y_i(x, s)$ be the set of length-$i$ strings such that for each $y \in Y_i(x, s)$, $y$ is a subsequence of $s$, $y$ starts and ends with the same bits as $x$, and $y[2:i-1]$ contains $x[2:k-1]$ as a subsequence. We write this as $Y_i(x)$ when $s$ is clear from context.
	\iscomment{show example}
	
	
	\iscomment{Do we need to define $\poly(n)$?}

==> results07-06.tex <==



% For a length $k$ substring $y$ of $s$, we derive an algorithm for estimating the following quantity 
% \al{
% K_{s,y,i} = \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{s_{j:j+k-1} = y \}.
% }
% $K_{s,y,i}$ is the probability that the beginning of a true copy of $y$ in $s$ gets shifted to position $i$ in a trace $\tilde{S}$ of $s$.  
% $K_{s,y,i}$ acts as a measure of density of the string $y$ in $s$, where $i/(1-p)$ is the position in $s$ that contributes most to $K_{s,y,i}$.
% We prove the following theorem about computing $K_{s,y,i}$ with at most $1/\text{poly}(n)$ error. %$K_{s,y,i}$ runs in polynomial time in $n$ if $k = c \log n$ for constant $c$ if $p < 0.5$.

Let $s \in \{0, 1\}^n $ denote the source string and $z \in \{0, 1\}^{k}$ denote the target $k$-mer, whose density $K_{s,z}$  we wish to estimate.


% Let $p$ denote the deletion probability.
\iscomment{I tried rewriting the main theorem a bit}


To simplify the notation, we fix a constant $c > 0$ and define 
\al{
f(n) = \frac{\left(1 + 2 n^{\alpha(p)}  \right)^2}{2 n^{2 c\log(1-p)-1}}
\quad \text{ and } \quad
\alpha(p) = 
    1 + c \log\left(\frac{1-p}{p}\right) + \frac{c H(1- \frac{p}{1-p})+\log\left(\frac{p}{1-p}\right)}{1- \frac{p}{1-p}}
    % + \frac{\log(p/(1-p))}{1 - p/(1-p)}
}
where $H(\cdot)$ is the binary entropy function.
The function $f(n)$ can be upper bounded by a polynomial of degree $\beta(c,p)$, which can be numerically computed as shown in Figure~\ref{fig:degree} \iscomment{can we compute this? maybe plot $\beta(c,p)$ as a function of $p$ for a few different values of $c$? Could be helpful later to make the case that, for small $p$, it is close to linear in $n$}


\begin{theorem} \label{thm:multibit}
    Suppose $p < 0.5$ and $k = c\log n$.
    Given
   $\log\left(\frac{2}{\delta}\right) \cdot \epsilon_n^{-2} \cdot f(n)
    $
    traces, an estimator $\hat K_{s,z}[i]$ for the $i$th entry of $K_{s,z}$ can be constructed so that $|\hat K_{s,z}[i] - K_{s,z}[i]| \leq \ep_n$ with probability $1-\delta$.
    Moreover, given $\log\left(\frac{2n^{1 + c\log 2}}{\delta}\right) \cdot \epsilon_n^{-2} \cdot f(n)$ traces, 
    an estimator for the entire density map $\hat K_s$ can be constructed so that $\|\hat K_s - K_s \|_\infty \leq \ep_n$ with probability $1-\delta$. 
\end{theorem}

\begin{oldtheorem} %\label{thm:multibit}
    Suppose $p < 0.5$ and $k = c\log n$, where $c$ is constant.
    With probability at least $1- \delta$, any entry of $K_{s,z}$ can be estimated with error at most $\epsilon_n$ using $\log(2/\delta) \frac{n}{2 \epsilon_n^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2$ traces where $f(p) = 1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}$. 
    Consequently, with probability at least $1- \delta$,  all entries of all vectors in the $k$-density map can be estimated with error at most $\epsilon_n$ using $\log(2n^{1 + c\log 2}/\delta) \frac{n}{2 \epsilon_n^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2$ traces.
\end{oldtheorem}
% \begin{theorem} \label{thm:multibit}
%     For $p < 0.5$ and $k = c\log n$ where $c$ is constant, with probability at least $1- \epsilon$, any entry of $K_{s,z}$ can be estimated with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$ 
%     Consequently, with probability at least $1- \epsilon$, for all $z$, all entries of $K_{s,z}$ can be estimated with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$ 
% \end{theorem}
In particular, Theorem~\ref{thm:multibit} implies that for $p < 0.5$ and $\epsilon_n = 1/g(n)$ where $g(n) \in  \text{poly}(n)$ \iscomment{better say $g(n) \in \poly(n)$?}, all entries of the $k$-mer density map $K_{s,z}$, for $k = c\log n$ can be estimated with error at most $\epsilon_n$ using $\poly(n)$ traces.

% Theorem \ref{thm:multibit} implies that for two strings $x, y \in \{0,1\}^n$, if there exists some choice of $z$ where $k = c\log n$ and index $i$ such that $|K_{x,z}[i] - K_{y,z}[i]| \geq \text{poly}(n)$, then $x$ can be distinguished from $y$ with high probability using $\text{poly}(n)$ traces.  This is stated formally in Corollary \ref{cor:distinguish_general}.

A consequence of Theorem~\ref{thm:multibit} is that source strings $s,s'$ whose ``density map distance'' $\| K_s - K_{s'} \|_\infty$ is not exponentially small in $n$ can be distinguished with $\poly(n)$ traces.
Hence, the trace reconstruction problem restricted to a set of binary strings with minimum density map distance $1/g(n)$ where $g(n) \in \poly(n)$ can be solved with $\poly(n)$ traces.

\begin{cor}
    \label{cor:distinguish_general}
    Suppose $p < 0.5$ and $k = c\log n$,
    % For $p < 0.5$ and $k = c\log n$ where $c$ is constant, 
    and let $\cA \subset \{0,1\}^n$ be such that, for any $s,s' \in \cA$, 
    \aln{
    \| K_s - K_{s'} \|_\infty \geq 2\ep_n. 
    }
    \iscomment{Do we need $2 \ep_n$ above?} \kmcomment{yes that makes sense}
    Given $\log\left(\frac{2n^{1 + c\log 2}}{\delta}\right) \cdot \epsilon_n^{-2} \cdot f(n)$ traces from some source string $s \in \cA$, $s$ can be correctly identified with probability $1-\delta$.
    % If the strings $x, y \in \{0, 1\}^n$ are such that for some $z \in \{0, 1\}^{c\log n}$ and index $i$, $|K_{x,z}[i] - K_{y,z}[i]| \geq 1/\text{poly}(n)$, then with probability $1-\delta$, $x$ can be distinguished from $y$ using $\text{poly}(n)$ traces.
\end{cor}

\iscomment{One additional point of discussion that we should include somewhere (maybe here) is that, with $\poly(n)$ traces, we can compute $\hat K_s$ for polynomially-many different values of $c$. Hence, we can distinguish sequences even if they are only different for one value of $c$}

\iscomment{I think we can maintain the discussion in terms of source strings $s$ and $s'$ instead of using $x$ and $y$ for that. It would be cleaner, and it would free up $x$ and $y$ to be substrings}

Recall that we can recover the $(c\log n)$-deck using $\text{poly}(n)$ traces with high probability as well, however, we can only distinguish between a pair of strings $s,s'$ using the $(c\log n)$-deck if $|\Vert K_{s, z}\Vert_1 - \Vert K_{s', z}\Vert_1| \geq 1$ for some $z$ since the number of times $z$ appears in $s$ is equal to $\Vert K_{s, z}\Vert_1$.  
Using Corollary \ref{cor:distinguish_general}, we can distinguish between a pair of strings $s,s'$ using $\text{poly}(n)$ traces if $\Vert K_{s, z} - K_{s', z} \Vert_\infty \geq 1/\text{poly}(n)$ for some $z\in \{0 ,1\}^{c\log n}$.  Also observe that due to the equivalence of $\ell_\infty$ norm and $\ell_0$ norm, and the reverse triangle inequality, we have that
\begin{align}
    \Vert K_{s, z} - K_{s', z} \Vert_\infty \geq \frac{1}{n} \Vert K_{s, z} - K_{s', z} \Vert_1 \geq \frac{1}{n} |\Vert K_{s, z}\Vert_1 - \Vert K_{s', z}\Vert_1|.
\end{align}
Thus if $ |\Vert K_{s, z}\Vert_1 - \Vert K_{s', z}\Vert_1| \geq 1/\text{poly}(n)$ for some $z$ where $k = O(\log n)$, then using the $k$-density map, we can distinguish $s$ from $s'$ with high probability using $\text{poly}(n)$ traces. This much less restrictive than distinguishing strings using the $k$-deck, further establishing the $k$-density map as a generalization of the $k$-deck.  It is not clear how to find an explicit string pair where the property in Corollary \ref{cor:distinguish_general} does not hold.  

A special case of Corollary \ref{cor:distinguish_general} with a simpler condition is given below.
% \begin{theorem} \label{thm:kdensity}
%     For $p < 0.5$ and $k = c\log n$ where $c$ is constant, the $k$-density map of $s$ can be estimated where each $K_{s,z,i}$ has error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$  
% \end{theorem}
\begin{cor}
    \label{cor:distinguish}
    For $p < 0.5$, if the strings $s, s' \in \{0, 1\}^n$ are such that $z \in \{0, 1\}^{k}$ begins at position $i$ in $s$ where $k = O(\log n)$ and, and $z$ does not appear in $s'$ at an index in the range $[i - n^{a}, i + n^{a}]$ for some $a > 0.5$, then $s$ can be distinguished from $s'$ with high probability using $\text{poly}(n)$ traces.
\end{cor}
Corollaries \ref{cor:distinguish_general} and \ref{cor:distinguish} are an addition to the set of results concerning distinguishing strings, which includes the facts that strings at constant Hamming distance can be distinguished using $\text{poly}(n)$ traces \cite{Mcgregor2014TraceRR}, \cite{Sudan}, and strings at constant Levenshtein distance can be distinguished using $\text{poly}(n)$ traces \cite{Bruck}.  Results similar to Corollaries \ref{cor:distinguish_general} and \ref{cor:distinguish} may be able to be obtained from \cite{chase}.

% Theorem \cite{thm:multibit} can also be used to visualize roughly where in $s$ each length $O(\log n)$ string appears. For each of the $2^{c\log n} = n^{c \log 2}$ possible kmers, we can compute $K_{s,y,i}$ for each of the  $n - k + 1$ possible positions $i$.  
% This yields a plot of the density of $y$ in $s$ for each possible $y$ using $\text{poly}(n)$ traces.   
% In addition, we can use $\text{poly}(n)$ traces to compute the $k$-deck of $s \in \{0,1\}^n$, defined as
% \al{
% \cS_k(s) = \{ s[i:i+k-1] : i =1,\dots,n-k+1 \},
% }
% i.e., the multi-set of all length-$k$ substrings of $s$.  Combining these two statistics, we have an understanding of roughly where copies of $y \in \cS_k(s)$ are located in $s$.
% put figure here

% \subsection{$k$-deck reconstruction}

\vspace{2mm}
\noindent {\bf Improved upper bound for $k$-deck reconstruction: \;}
Using our proof technique for estimating $K_{s,z}$, we also give a novel proof that the $(c\log n)$-deck where $c$ is constant can be reconstructed using $\text{poly}(n)$ traces for $p < 0.5$ which we discovered independently in 2021, and improve the upper bound \cite{Servedio} on the number of traces for reconstructing the ($c\log n$)-deck of a string for $p < 0.5$ .  

\begin{theorem}
    For deletion probability $p < 0.5$, and any source string $s \in \{0,1\}^n$, we can reconstruct the $(c\log n)$-deck with high probability using
    \al{
     O\left(\log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right)
    }
    traces.
\end{theorem}
The analysis in \cite{Servedio2} proves that 
\al{O\left(n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)}\right)}
traces are sufficient for this task. 
Clearly, the the upper bound we obtain is smaller for $p$ that is not too close to $0$.
% add statement here about how small p needs to be for existing bound to be better.
Using the lower bound we derive below, we see that as $c$ gets close to $0$, our upper bound becomes optimal up to log factors. 
	\begin{theorem}
	    For deletion probability $p$ and any source string $s \in \{0, 1\}^n$, we have that $\Omega(n p (1-p))$ traces are necessary for recovering the $f(n)$-spectrum for any function $f$ such that $f(n) \geq 2$.
	\end{theorem}
	
	\begin{IEEEproof}
	    Suppose we want to decide whether the $k$-deck of the source string is the $k$-deck of $s_1 = 1^{n/2} 0^{n/2}$, or whether it is the $k$-deck of $s_2 = 1^{(n/2) + 1} 0^{(n/2 -1}$.  Observe that for any $k \geq 2$, the only length $n$ string that has the $k$-deck of $s_1$ is $s_1$ itself, and likewise, the only length $n$ string that has the $k$-deck of $s_2$ is $s_2$ itself.  Thus, distinguishing between these two $k$-decks is equivalent to distinguishing between $s_1$ and $s_2$.  From Section 4.2 of \cite{Batu}, we know that $\Omega(n p (1-p))$ traces are necessary for distinguishing between $s_1$ and $s_2$.
	\end{IEEEproof}	    
    We also show that truncating the polynomial in the algorithm from \cite{Servedio} for reconstructing the ($\log n$)-deck  is not necessary to prove that $\text{poly}(n)$ traces suffice for reconstructing the ($\log n$)-deck of a string for $p < 0.5$.

%prove that $\text{poly}(n)$ traces suffice for trace reconstruction in the smoothed complexity model.

% The $k$-deck is a common object of interest in sequence reconstruction problems in bioinformatics~\cite{euler,yaakobi,errorcorrection}.
% In particular, a classical result by Ukkonen~\cite{ukkonen} provides necessary and sufficient conditions for when $\cS_k(s)$ uniquely determines $s$.
% Hence, the $k$-spectrum can be thought of as an intermediate step towards the reconstruction of $s$.  

% 	\subsection{Prior Work}
	
% 	The trace reconstruction problem was first introduced as the sequence reconstruction problem by Levenshtein in 2001 \cite{Lev1}, \cite{Lev2}, where he studied the how many distinct traces of a certain length are necessary in the worst case to reconstruct any source string.  This differs from our setup because the sample complexity required for reconstruction is studied for the worst case set of traces of a given length, i.e. no randomness is used in the generation of the traces.   
    
%     The first study of trace reconstruction where the traces are randomly generated was published in 2004 by Batu, Kannan, Khanna, and McGregor \cite{Batu} where they provided an algorithm that reconstructs a uniformly random source string with high probability using $O(\log(n))$ traces where the deletion probability is $p = O(1/\log(n))$.  The uniformly random source string case was subsequently improved in numerous papers, and currently, the best known algorithm was presented by Holden, Permantle, and Peres.  Their algorithm and uses $\exp(O(\log^{1/3} (n)))$ traces for any deletion probability $p \in [0, 1)$.  Interestingly, their algorithm also handles any constant insertion probability in the range $[0, 1)$.
    
%     The first result on trace reconstruction with random traces for a worst case source string also appeared in \cite{Batu} where they showed that a variation of their algorithm for a random source string reconstructs a worst case source string with high probability using $O(n\log(n))$ traces for deletion probability $p = O(1/n^{1/2 + \epsilon})$.
%     The current best result for reconstructing the worst case source string with constant deletion probability $p \in [0, 1)$ was published in 2021 by Chase where $\exp(\tilde{O}(n^{1/5}))$ traces are used. 
    
    
% \subsection{Our Results}

% \begin{theorem}
%     For $p < 0.5$ and any source string $s \in \{0, 1\}^n$, target string $z \in \{0, 1\}^{k}$ where $k = c\log n$ and $c$ is constant, and index $i$, we can estimate $K_{s,z,i}$ with error at most $1/f(n)$ using $\text{poly}(n)$ traces if $f(n) = O(\text{poly}(n)).$  
% \end{theorem}
% \begin{cor}
%     For $p < 0.5$, if $x \in \{0, 1\}^n$ and $y \in \{0, 1\}^n$ are such that $z \in \{0, 1\}^{k}$ begins at position $i$ in $x$ where $k = O(\log n)$ and, and $z$ does not appear in $y$ at an index in the range $[i - n^{a}, i + n^{a}]$ for some $a > 0.5$, then $x$ can be distinguished from $y$ using $\text{poly}(n)$ traces.
% \end{cor}
% \begin{theorem}
%     For deletion probability $p < 0.5$, and any source string $s \in \{0,1\}^n$, we can reconstruct the $c\log n$-spectrum with high probability using
%     \al{
%      O\left(log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right)
%     }
%     traces.
% \end{theorem}
% The analysis in \cite{Servedio2} proves that 
% \al{O\left(n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)}\right)}
% traces are sufficient for this task.  
% Clearly, the the upper bound we obtain is smaller for $p$ that is not too close to $0$.
% % add statement here about how small p needs to be for existing bound to be better.
% Using the lower bound we derive below, we see that as $c$ gets close to $0$, our upper bound becomes optimal up to log factors. 
% 	\begin{theorem}
% 	    For deletion probability $p$ and any source string $s \in \{0, 1\}^n$, we have that $\Omega(n p (1-p))$ traces are necessary for recovering the $f(n)$-spectrum for any function $f$ such that $f(n) \geq 2$.
% 	\end{theorem}
	
% 	\begin{IEEEproof}
% 	    Suppose we want to decide whether the $k$-spectrum of the source string is the $k$-spectrum of $s_1 = 1^{n/2} 0^{n/2}$, or whether it is the $k$-spectrum of $s_2 = 1^{(n/2) + 1} 0^{(n/2 -1}$.  Observe that for any $k \geq 2$, the only length $n$ string that has the $k$-spectrum of $s_1$ is $s_1$ itself, and likewise, the only length $n$ string that has the $k$-spectrum of $s_2$ is $s_2$ itself.  Thus, distinguishing between these two $k$-spectrums is equivalent to distinguishing between $s_1$ and $s_2$.  From Section 4.2 of \cite{Batu}, we know that $\Omega(n p (1-p))$ traces are necessary for distinguishing between $s_1$ and $s_2$.
% 	\end{IEEEproof}	    

% 	%Unfortunately, the pair of strings used in  \cite{Chase2} for the best known lower bound for worst case trace reconstruction have the same $k$-spectrum for many interesting values of $k$.  


	
\section{An Estimator for $k$-mer Density Map}

For strings $x, y$, let $\binom{y}{x}' = \binom{y[2:-2]}{x[2:-2]}$. For a string $x$, let $Y_i(x, s)$ be the set of length-$i$ strings such that for each $y \in Y_i(x, s)$, $y$ is a subsequence of $s$, $y$ starts and ends with the same bits as $x$, and $y[2:-2]$ contains $x[2:-2]$ as a subsequence. For example, if $x = 101$ and $s = 101010001$, then $Y_5(x,s) = \{10101, 10001\}$.
We write this as $Y_i(x)$ when $s$ is clear from context.  



For source string $s$ and length $k$ string $x$, let $E_{s, x, i} = E[\mathbbm{1}\{\tilde{S}[i:i+|z|-1] = z \}]$, and recall that
\al{
K_{s,x}[i] = \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{\tilde{S}[j:j+\ell-1] = x \}.
}
The first part of the proof is a derivation of the following formula
\al{
    K_{s, x, i} = \frac{1}{(1-p)^k}\left( E_{x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_{y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right).
}
This formula for $K_{s, x, i}$ depends only on $E_{s, y, i}$ for all strings $y$, so $K_{s, x, i}$ can be estimated from the easily computable estimates of $E_{s, y, i}$.  Our estimator for $K_{s, x, i}$ is given by
\al{
    \hat{K}_{s, x, i} = \frac{1}{(1-p)^k}\left( \hat{E}_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_{s, y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right)
}
where $\hat{E}_{s, x, i} = \frac{1}{T} \sum_{t = 1}^T \mathbbm{1}\{\tilde{S}_t[i:i+|x|-1] = x \}$.
We then use McDiarmid's inequality to understand how many traces are needed for this estimator of $K_{s, x, i}$ to perform at a certain level of accuracy with high probability.  

To derive our formula for $\hat{K}_{s, x, i}$, we begin by deriving a recursive estimator for $\hat{K}_{s, x, i}$.  We have
\al{
    E_{s, x, i} & = \sum_{\ell = k}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k \sum_{j=i}^n \binom{j-1}{i-1} (1-p)^{i-1} p^{j-i} \mathbbm{1}\{\tilde{s}_{j:j+\ell-1} = y \}
    \\ & = \sum_{\ell = k}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k K_{s, y, i}.
}
This can be rewritten as the recursive formula
\al{
    K_{s, x, i} & = \frac{1}{(1-p)^k} 
    \left( E_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_\ell(x)} \binom{y}{x}' p^{\ell - k} (1-p)^k K_{s, y, i} \right)
    \\ & = \frac{1}{(1-p)^k} 
    \left( E_{s, x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_\ell(x)} (1-p)^\ell \binom{y}{x}'  K_{s, y, i} \left(\frac{p}{1-p}\right)^{\ell - k} \right).
}
This recursive formula can be expanded so that $K_{s, x, i}$ is written only in terms of $E_{s, x, i}$.  
This yields a formula of the form
\begin{align}
	K_{s, x, i} = \frac{1}{(1-p)^k} \left(E_{s, x, i} - \sum_{\ell=k+1}^n \sum_{y \in Y_\ell(x)} E_{s, y, i} a_{y, x, s} \left(\frac{ p}{1-p}\right)^{\ell-k} \right)
\end{align}
where $a_{y, x, s} \in \mathbb{Z}$ is a constant that depends on $y, x, s$.
Observe that $a_{y, x, s}$ obeys the following recursion:  for $y \in Y_\ell(x)$, we have that 
\begin{align}
	a_{y,x,s} = \binom{y[2:-2]}{x[2:-2]} - \sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x)} a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}. 
\end{align}
This is because as we expand the recursive formula for $K_{s, x, i}$ one step at a time, we observe that every time we obtain a new term involving $E_{s, y, i}$ in the expansion with coefficient $c_y \left(\frac{p}{1-p}\right)^{|y| - k}$, at the next step of the expansion we obtain a term involving $E_{s, z, i}$ with coefficient $-c_y \binom{z[2:-2]}{y[2:-2]} \left(\frac{p}{1-p}\right)^{|z| - k}$ for every $z \in \cup_{\ell = |y| + 1}^n Y_\ell(y)$.

We proceed to prove that for any $x$, $y$, $s$, we then have that 
\begin{align}
	a_{y,x,s} = (-1)^{|y| -|x|+1} \binom{y[2:-2]}{x[2:-2]}.
\end{align}
If $|y| - |x| = 1$, this clearly holds.  
Suppose it holds for $|y| - |x| <  m$.  Then if $|y| - |x| =  m$, we have that
\begin{align}
	a_{y,x,s} & = \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}
	\\ & =  \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| -|x| + 1} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
	\\ & =  \binom{y[2:-2]}{x[2:-2]} + 	\sum_{k+1 \leq j < \ell} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| + |x|} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
	\\ & = \binom{y[2:-2]}{x[2:-2]} + \left(- \binom{y[2:-2]}{x[2:-2]} - (-1)^{|y| + |x|} \binom{y[2:-2]}{x[2:-2]}\right)
	\\ & =  (-1)^{|y| - |x| + 1} \binom{y[2:-2]}{x[2:-2]}.
\end{align}	
where the fourth line follows from Corollary (6.3.9) in \cite{Lothaire}, 
which states that 
for some alphabet $\Sigma$ and all strings $f, g$ we have
\begin{align}
    \sum_{h} (-1)^{|g| + |h|} \binom{f}{h} \binom{h}{g} = \delta_{f, g}
\end{align}
where $\delta_{f, g} = 0$ if $f \neq g$, and $\delta_{f, g} = 1$ if $f = g$.
Therefore, we can write $K_{s, x, i}$ only in terms of the terms $E_{s, y, i}$ for all $y$:
\al{
    K_{s, x, i} = \frac{1}{(1-p)^k}\left( E_{x, i} - \sum_{\ell = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_{y, i} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k} \right).
}

\subsection{sample complexity analysis}
Changing a single bit in the $t$th trace $\tilde{S}_t$ changes the estimator by at most
\begin{align}
    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + \sum_{\ell = k+1}^n 2 \max_{y \in Y_\ell (x)} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left(1 + \sum_{\ell = k+1}^n 2  \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right).
\end{align}
%For $k = c\log(n)$ for constant $c$ and $p < 0.5$, 
To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
\begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( 1 + 2 n \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{\ell-c\log(n)}\right)
\\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( 1 + 2 n \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell-c\log(n)}\right)
\\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{1 + c \log(\frac{1-p}{p})}  \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell}\right).
\end{align}
where we take $\log()$ to have base 2. 
We have that
\begin{align}
    & \max_{\ell \in [c\log(n)+1, n]}  \binom{\ell}{c\log(n)} \left(\frac{p}{1-p}\right)^{\ell}
    \\ & \leq \max_{\ell \in [c\log(n)+1, n]} 2^{\ell H(c\log(n)/\ell)} \left(\frac{p}{1-p}\right)^{\ell}
    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
\end{align}
because the maximizing $\ell$ is given by $\ell^* = \frac{\log(n^c)}{1- p/(1-p)}$ .
This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
\begin{align}
    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
\end{align}
where $q = p/(1-p)$,
the function is a differentiable for $x \in (c\log(n)+1, n),$
and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
\begin{align}
    - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
\end{align}
which is negative.
We therefore have that we  have that 
\begin{align} 
    b &
    \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{1 + c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
\end{align}    
when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
Let
\begin{align}
    f(p) = 1 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
\end{align}
Plugging this into McDiarmid's inequality,  we have
\begin{align}
	\Pr \left(|\hat{K}_{s,x,i} - K_{s,x,i}| \geq \epsilon \right) & \leq 2\exp \left(-\frac{2\epsilon^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{f(p)}  \right) \right)^2}\right)
	\\ & = 2\exp \left(-\frac{2T\epsilon^2}{n \left(\frac{1}{n^{c\log(1-p)}}\left( 1 + 2 n^{f(p)}  \right)\right)^2}\right)
\end{align}
Setting $\delta = \Pr \left(|\hat{K}_{s,x,i} - K_{s,x,i}| \geq \epsilon \right)$, we have
\begin{align}
    T = \log(2/\delta) \frac{n}{2\epsilon^2} \left(\frac{1}{n^{c\log(1-p)}}\left(1 + 2 n^{f(p)}  \right)\right)^2
\end{align}
traces suffices for recovering $K_{s,x,i}$ with error $< \epsilon$ with probability at least $1 - \delta$.

% \subsection{analysis for $k = c\sqrt{n}$}

% Using McDiarmid's inequality as before, we have that changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
% \begin{align}
%     b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + \sum_{\ell = k+1}^n 2 \max_{y \in Y_\ell (x)} \binom{y}{x}' \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left(1 + \sum_{\ell = k+1}^n 2  \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell-2}{k-2} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   \binom{\ell}{k} \left(\frac{p}{1-p}\right)^{\ell-k}\right)
%     \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( 1 + 2 n \max_{\ell \in [k+1, n]}   2^{\ell H(k/\ell)} \left(\frac{p}{1-p}\right)^{\ell-k}\right).
% \end{align}
% For $k = c\sqrt{n}$, we have 
% \al{
%     \frac{d}{d\ell} 2^{\ell H(k/\ell)} \left(\frac{p}{1-p}\right)^{\ell-k} = \left(\frac{p}{1-p}\right)^{\ell - \sqrt{n}} \left(1 - \frac{\sqrt{n}}{\ell}\right)^{\sqrt{n} - \ell} \left(\frac{\sqrt{n}}{\ell}\right)^{-\sqrt{n}} \left(\log(\frac{p}{1-p}) -  \log(1 - \frac{\sqrt{n}}{\ell})\right)
% }
% Let $q = \frac{p}{1-p}$. Setting the derivative equal to zero and solving for $\ell$, we obtain 
% \al{
%     \ell^* = \frac{\sqrt{n}}{1 - q}.
% }
% Plugging this in, we obtain
% \al{
%     q^{\sqrt{n}\frac{q}{1 - q}} 2^{\frac{\sqrt{n} ((q - 1) \log(1 - q) - q \log(1 - \sqrt{n} (1 - q)))}{(1 - q) \log(2)}}.
% }

	\section{$K$-deck Reconstruction}
	
	In order to recover the $k$-spectrum for source string $s$ and deletion probability $p$, we need to estimate $N_x$ for each of the possible $2^k$ strings of length $k$.  However, it is not immediately clear how to construct an estimator $\hat{N}_x$. Our approach is to first write $N_x$ in terms of $E_y$ for all strings $y \in \cup_{i = k+1}^n Y_i(x)$.  $E_y$ is easily estimated as $\hat{E}_y = \frac{1}{T}\sum_{i = 1}^T (\text{\# of times $y$ appears as a substring in trace $t_i$})$, which we subsequently plug into the formula we derive for $N_x$ in order to form our estimate $\hat{N}_x$.

    Our estimator is given by
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	\end{align}
	which we then round to the nearest integer.  Observe that if the error in the estimate of $N_x$ is $< 1/2$, then we will estimate $N_x$ correctly after rounding.
	
	For any $k$, our estimator can be computed in $O(T n^2 \binom{n}{k})$ time because for each of the $T$ traces, we need to compute $\binom{y[2:-2]}{x[2:k-1]}$ for each of the $O(n^2)$ substrings in the trace, and computing $\binom{y[2:-2]}{x[2:k-1]}$ using a brute force approach takes $O(\binom{n}{k})$ time.

    In order to derive our estimator, we begin by writing a recursive formula for $N_x$ which we subsequently use to obtain a nonrecursive formula for $N_x$ in terms of $E_y$s.  This nonrecurive formula yeilds our estimator.
	

	
	\begin{theorem} \label{theorem:rec_estimator}
	    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
		\begin{align}
			N_x = \frac{1}{(1-p)^k}\left(E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} (1-p)^i N_{y} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
		\end{align}  
	\end{theorem}	
	
	\begin{IEEEproof}
		In this proof, let $E_{\hat{z}} = (1-p)^{|z|} N_z$ i.e. $E_{\hat{z}}$ is the expected number of times a copy of $z$ (contained as a substring of $s$) is unaffected by deletions in a trace.  $E_{\hat{z}} = 0$ if and only if $z$ is not a substring of $s$.   Observe that $E_{\hat{x}}$ is equal to $E_x$ minus the expected number of copies of $x$ that appear in the trace due to deletions.  This follows from linearity of expectation applied to the indicator random variables that copies of $x$ are formed using bits at specific positions in $s$ as the start and end bits of the copies of $x$.
		Any copy of $x$ in a trace that is formed from deletions is created by  deleting elements at internal positions in some $y \in Y_i(x)$ for some $i > k$ that is a true copy of $y$ in $s$.
		For a  particular $i \in \mathbb{N}$, we have that for a position $r$ in $s$ such that $ s[r:r+i-1] = y \in 
		Y_i(x)$, the expected value of the indicator random variable that a copy of $x$ is formed using the start and end bits of $s[r:r+i-1]$ is given by $(1-p)^i \binom{y[2:i-1]}{x[2:k-1]}\frac{ p^{i - k}}{(1-p)^{i-k}}$.  If there are $c$ such positions $r$ for this $y$, we have that the expected number of times $x$ arises using these pairs of bits as the start and end bits in the copy of $x$ is given by   
		\begin{align}
			E_{\hat{y} \to x} = c \binom{y[2:-2]}{x[2:-2]} (1-p)^k p^{i - k} = c (1-p)^i \binom{y[2:-2]}{x[2:-2]} \frac{ p^{i - k}}{(1-p)^{i-k}} = E_{\hat{y}} \binom{y[2:-2]}{x[2:-2]} \frac{ p^{i - k}}{(1-p)^{i-k}}
		\end{align} by applying linearity of expectation to the sum of the indicator random variables for the terms corresponding to each copy of $y$ in $s$.   
		Then summing over all $y \in Y_i(x)$ for all valid $i$, we are left with  
		\begin{align}
			\sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{\hat{y}} \binom{y[2:i-1]}{x[2:k-1]} \frac{ p^{i - k}}{(1-p)^{i-k}}.
		\end{align}  
		by linearity of expectation.
		Thus, we have
		\begin{align}
			E_{\hat{x}} = E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{\hat{y}} \binom{y[2:i-1]}{x[2:k-1]} \frac{ p^{i - k}}{(1-p)^{i-k}}.
		\end{align} 
		%For the largest value of $i$ such that $Y_i(x) \neq \emptyset$, There is clearly only one element in $Y_i(x)$, and there is no way to form this $y$ from deletions so $E_{\hat{y}} = E_{y}$.
	\end{IEEEproof}

	
	\begin{theorem} \label{theorem:estimator}
	    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
	    \begin{align}
	        N_x = \frac{1}{(1-p)^k}\left( E_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	    \end{align}
	\end{theorem}	
	
	\begin{IEEEproof}
	    We can expand the recursion in Theorem \ref{theorem:rec_estimator} so that $N_x$ is only written in terms of $E_y$s. 
	    The resulting formula will be of the following form
    	\begin{align}
    		N_{x} = \frac{1}{(1-p)^k} \left(E_x - \sum_{i=k+1}^n \sum_{y \in Y_i(x)} E_{y} a_{y, x, s} \left(\frac{ p}{1-p}\right)^{i-k} \right)
    	\end{align}
    	where $a_{y, x, s} \in \mathbb{Z}$ is a constant that depends on $y, x, s$.
    	We observe that $a_{y, x, s}$ obeys the following recursion:  for $y \in Y_i(x)$, we have that 
    	\begin{align}
    		a_{y,x,s} = \binom{y[2:-2]}{x[2:-2]} - \sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x)} a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}. 
    	\end{align}
    	This is because as we expand the recursive formula for $N_x$ one step at a time, we observe that every time we obtain a new term involving $E_y$ in the expansion with coefficient $c_y \left(\frac{p}{1-p}\right)^{|y| - k}$, at the next step of the expansion we obtain a term involving $E_z$ with coefficient $-c_y \binom{z[2:-2]}{y[2:-2} \left(\frac{p}{1-p}\right)^{|z| - k}$ for every $z \in \cup_{i = |y| + 1}^n Y_i(y)$.
    	
    	We proceed to prove that for any $x$, $y$, $s$, we then have that 
		\begin{align}
			a_{y,x,s} = (-1)^{|y| -|x|+1} \binom{y[2:-2]}{x[2:-2]}.
		\end{align}
		If $|y| - |x| = 1$, this clearly holds.  
		Suppose it holds for $|y| - |x| <  m$.  Then if $|y| - |x| =  m$, we have that
		\begin{align}
			a_{y,x,s} & = \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } a_{z,x,s} \binom{y[2:-2]}{z[2:-2]}
			\\ & =  \binom{y[2:-2]}{x[2:-2]} - 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| -|x| + 1} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
			\\ & =  \binom{y[2:-2]}{x[2:-2]} + 	\sum_{k+1 \leq j < i} \;\; \sum_{z : \; z \in Y_j(x), } (-1)^{|z| + |x|} \binom{z[2:-2]}{x[2:-2]} \binom{y[2:-2]}{z[2:-2]}
			\\ & = \binom{y[2:-2]}{x[2:-2]} + \left(- \binom{y[2:-2]}{x[2:-2]} - (-1)^{|y| + |x|} \binom{y[2:-2]}{x[2:-2]}\right)
			\\ & =  (-1)^{|y| - |x| + 1} \binom{y[2:-2]}{x[2:-2]}.
		\end{align}	
		where the fourth line follows from Corollary (6.3.9) in \cite{Lothaire}, 
		which states that 
		for some alphabet $\Sigma$ and all strings $f, g$ we have
		\begin{align}
		    \sum_{h} (-1)^{|g| + |h|} \binom{f}{h} \binom{h}{g} = \delta_{f, g}
		\end{align}
		where $\delta_{f, g} = 0$ if $f \neq g$, and $\delta_{f, g} = 1$ if $f = g$.
	\end{IEEEproof}

    \section{Analysis of Estimator (Improved and Simplified)}
	McDiarmid's inequality states the following.  Let $X_1, ..., X_m$ are iid random variables. Suppose the function $f$ has the property that for any sets of values $x_1, x_2, ..., x_m$ and $x'_1, x'_2, ..., x'_m$ that only differ at the $i$th random variable, it follows that 
	\begin{align}
		&
		|f(x_1, x_2, ..., x_m) - f(x'_1, x'_2, ..., x'_m)| \leq b_i.
	\end{align} 
	Then, for any $t > 0$, we have that 
	\begin{align}
		\Pr(f(X_1, X_2, ..., X_m) - \mathbb{E}[f(X_1, X_2, ..., X_m)] \geq t) \leq \exp \left(-\frac{2t^2}{\sum_{i = 1}^m b_i^2}\right). 
	\end{align}
	Applying this to our problem, we set $f = \hat{N}_x$ and we take each random variable $X_i$ to be an indicator of whether a particular bit in $s$ is deleted in a particular trace.  
	
    Recall that our estimator is given by 
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
	\end{align}
	Changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
	\begin{align}
	    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( \min(k, n-k+1) + \sum_{i = k+1}^n 2 \min(i, n-i+1) \max_{y \in Y_i (x)} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + \sum_{i = k+1}^n 2 i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 n \max_{i \in [k+1, n]} i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 n^2 \max_{i \in [k+1, n]}  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	\end{align}
	To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
    \begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 n^2 \max_{i \in [c\log(n)+1, n]}  \binom{i-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 n^2 \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log(\frac{1-p}{p})}  \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}\right).
	\end{align}
	where we take $\log()$ to have base 2. 
	We have that
	\begin{align}
	    & \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq \max_{i \in [c\log(n)+1, n]} 2^{i H(c\log(n)/i)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
	    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
	\end{align}
	The maximizer is given by $i = \frac{\log(n^c)}{1- p/(1-p)}$ .
	This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
	\begin{align}
	    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
	\end{align}
	where $q = p/(1-p)$,
	the function is a differentiable for $x \in (c\log(n)+1, n),$
	and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
	\begin{align}
        - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
	\end{align}
    which is negative.
    We therefore have that 
        \begin{align} b &
        \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
        \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
	\end{align}    
    when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
    Let
    \begin{align}
        f(p) = 2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
    \end{align}
	Plugging this into McDiarmid's inequality, and setting $\epsilon = 1/2$,  we have
	\begin{align}
		\Pr \left(\hat{N}_x - N_x \geq \frac{1}{2} \right) & \leq \exp \left(-\frac{2\left( \frac{1}{2}\right)^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right) \right)^2}\right)
		\\ & = \exp \left(-\frac{T}{2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2}\right)
    \end{align}
    Setting $\delta = \Pr \left(\hat{N}_x - N_x \geq \frac{1}{2} \right)$, we have
    \begin{align}
        T = \log(1/\delta) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2
    \end{align}
    traces suffices for recovering $N_x$ with probability at least $1 - \delta$.

	There are $2^{c\log(n)}$ strings $x$ in total to test, so if we want to upper bound the probability of making making a mistake in estimating any $x$ using the number of traces above, we can use the union bound. Setting $\delta = \frac{1}{n2^{c\log(n)}}$, we have
    \begin{align}	
        T & \sim \log(n2^{c\log(n)})2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = \log(e^{log(n)+ c\log(n) \log(2)}) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = 2n (log(n)+ c\log(n) \log(2))  \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)} \right)\right)^2
        \\ & = O(\text{poly}(n)).
    \end{align}	
    traces suffice. 
    
    Using the union bound on the probability of error over all $2^{c\log(n)}$ kmers, we get a probability of error upper bounded by
	\begin{align}
		2^{c\log(n)} \frac{1}{n2^{c\log(n)}} = \frac{1}{n}.
	\end{align}
	Thus for $p \in [0, .5)$, we reconstruct the  the $c\log(n)$-spectrum of $s$ with probability greater than $1 - \frac{1}{n}$ using $O(\text{poly}(n))$ traces.  	


\section{Comparison with results from Servedio paper}

\subsection{Difference in Techniques}
Recall that our main structural result is the following theorem.
\begin{theorem} 
    For source string $s \in \{0, 1\}^n$, deletion probability $p \in [0, 1)$, and $x \in \{0, 1\}^k$, we have  
    \begin{align}
        N_x = \frac{1}{(1-p)^k}\left( E_x - \sum_{i = k+1}^n \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} E_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right).
    \end{align}
\end{theorem}	
To estimate $N_x$ for $p < 0.5$, we  directly estimate $ E_y$ from the traces and calculate $\binom{y[2:i-1]}{x[2:k-1]}$ for $y \in Y_i(x), \;  i \geq k$.
In the Servedio paper, they first present an algorithm for $p < 0.5$ where they instead estimate $E[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, y)]$ from the traces and estimate $N_x$ using the formula 
\al{
    N_x = \frac{1}{(1-p)^k} \sum_{\substack{\alpha \in \mathbb{Z}_{\geq 0}^{k-1} \\ |\alpha| \leq n-k}} E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right] \left(\frac{-p}{1-p}\right)^{|\alpha|}
}
where $*$ is the wildcard symbol and $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)$ is the number of times a substring of the form $x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}$ appears in a trace $t$ of $s$ with deletion probability $p$, and $|\alpha| = \sum_{i=1}^{k-1} |\alpha_i|$ for $\alpha \in \mathbb{Z}_{\geq 0}^{k-1}$.
Observe that we derived the same polynomial as the Servedio paper but in a different form.  Our proof is very different from theirs in that we first derive a recursive estimator of $N_x$ and then use structural knowledge of $\binom{y[2:i-1]}{x[2:k-1]}$ to prove its equivalence to the polynomial above.

In their initial algorithm for $p < 0.5$, they just bound the error of the estimate of each $ E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right]$ using a Chernoff bound and the fact that $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t) \in [0, n]$.  For this reason, their initial algorithm for calculating $N_x$ where $|x| = k$ for $p < 0.5$ uses $n^{O(k)} \cdot \log(1/\delta)$ traces and running time.  For $k = c \log(n)$ which is what both their paper and our paper are interested in, their number of traces and running time is superpolynomial  in $n$ whereas ours is polynomial in $n$.  

In their improved algorithm for $p < 0.5$ that uses polynomial runtime and number of traces in $n$, they estimate $N_x$ using only estimates of $E_y$ for substrings $y$ of length at most $d + k$ where $d := \frac{e^2}{1/2 - \delta} \left( k\log \left(\frac{e^2}{1/2 - \delta}\right) + \log(n) \right)$.  The formula they use is then
\al{
    N_x = \frac{1}{(1-p)^k} \sum_{\substack{\alpha \in \mathbb{Z}_{\geq 0}^{k-1} \\ |\alpha| \leq d}} E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right] \left(\frac{-p}{1-p}\right)^{|\alpha|}.
}
They then prove that the sum of the terms in the polynomial for strings $y$ of length $>d+k$ are small and they again bound the error of the estimate of each $ E \left[\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t)\right]$ using a Chernoff bound and the fact that $\#(x_0 *^{\alpha_1} x_1 *^{\alpha_2} x_2 \cdot \cdot \cdot  x_{k-2} *^{\alpha_{k-1}} x_{k-1}, \; t) \in [0, n]$. 

This is different from our analysis because we don't truncate the polynomial, and we use McDiamids inequality to bound the error in the entire polynomial instead of using a Chernoff bound to  bound to the error of the estimate of each coefficient in the polynomial followed by a union bound.  


\subsection{Comparison of Results}

In the Serverdio paper, the number of traces used by their algorithm to recover $N_x$ with probability at least $1- \delta$ for $p < 1/2$ is
\begin{align}
    O((M^2 2^k)^2) \log\left(\frac{M}{\delta}\right) & = O\left( \left( \left(n \left(\frac{e^2}{1/2 - p}\right)^{3k} \right)^2 2^k\right)^2\right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3k}}{\delta}\right)
    \\ & = O\left( n^4  \left(\frac{e^2}{1/2 - p}\right)^{12k}  4^k \right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3k}}{\delta}\right).
\end{align}
For $k = c \log(n)$, we have that the number of traces used is
\begin{align}
    & O\left( n^4  \left(\frac{e^2}{1/2 - p}\right)^{12c\log(n)}  4^{c\log(n)} \right) \log\left(\frac{n \left(\frac{e^2}{1/2 - p}\right)^{3c\log(n)}}{\delta}\right)
    \\ & = O\left( n^4  n^{12c \left(\frac{e^2}{1/2 - p}\right)}   n^{c\log(4)} \right) \log\left(\frac{n \cdot n^{3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right)
    \\ & = O\left( n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)} \right) \log\left(\frac{n^{1 + 3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right)
    \\ & = O\left( n^{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4)} \right) \log\left(\frac{n^{1 + 3c\log\left(\frac{e^2}{1/2 - p}\right)}}{\delta}\right).
\end{align}
In comparison, the number of traces used by our algorithm for recovering $N_x$ with probability at least $1- \delta$ for $p < 1/2$ is
\begin{align}
    & \log(1/\delta) 2n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 n^{f(p)}  \right)\right)^2
    \\ & = O \left(n^{1 + 2 \left(f(p) + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
\end{align}
traces where
\begin{align}
    f(p) & = 2 + c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}.
\end{align}
Observe that we can upper bound $f(p)$ as follows
\begin{align}
    f(p)  \leq 2 + c \log((1-p)/p) + \frac{c }{1- p/(1-p)}
\end{align}
by using the fact that $H(x) \leq 1$ for all $x$ and $\log(p/(1-p)) < 0$ for $p < 0.5$. 
Thus, the number of traces needed by our algorithm is upper bounded by 
\begin{align}
    & O \left(n^{1 + 2 \left(2 + c \log((1-p)/p) + \frac{c }{1- p/(1-p)} + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
    \\ & = O\left(n^{5 + 2 c \log((1-p)/p) + \frac{2c }{1- p/(1-p)} + 2c\log\left(\frac{1}{1-p}\right)}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c (\log(1/p) + \frac{1 }{1- p/(1-p)})}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c (\log(1/p) + \frac{1-p}{1-2p})}  \right)\log(1/\delta)
    \\ & = O\left(n^{5 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)\log(1/\delta).
\end{align}
Recall that the exponent of $n$ in the number of traces used by Servedio's algorithm is 
\al{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4).}
Clearly, the number of traces used by our algorithm is smaller for $p$ close to $0.5$ and $c=1$ which is the $c$ they used in their paper.

\section{Analysis of Truncated Estimator}
	McDiarmid's inequality states the following.  Let $X_1, ..., X_m$ are iid random variables. Suppose the function $f$ has the property that for any sets of values $x_1, x_2, ..., x_m$ and $x'_1, x'_2, ..., x'_m$ that only differ at the $i$th random variable, it follows that 
	\begin{align}
		&
		|f(x_1, x_2, ..., x_m) - f(x'_1, x'_2, ..., x'_m)| \leq b_i.
	\end{align} 
	Then, for any $t > 0$, we have that 
	\begin{align}
		\Pr(f(X_1, X_2, ..., X_m) - \mathbb{E}[f(X_1, X_2, ..., X_m)] \geq t) \leq \exp \left(-\frac{2t^2}{\sum_{i = 1}^m b_i^2}\right). 
	\end{align}
	Applying this to our problem, we set $f = \hat{N}_x$ and we take each random variable $X_i$ to be an indicator of whether a particular bit in $s$ is deleted in a particular trace.  
	
    Recall that the truncated estimator from the Servedio paper written in our form is given by 
    \begin{align}
        \hat{N}_x = \frac{1}{(1-p)^k}\left( \hat{E}_x - \sum_{i = k+1}^d \sum_{y \in Y_i (x)} (-1)^{|y| - |x| + 1} \hat{E}_y  \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k} \right)
	\end{align}
	where 
	\begin{align}
	    d = \frac{e^2}{1/2 - p} \left( k \ln \frac{e^2}{1/2 - p} + \ln n \right).
	\end{align}
	Changing a single bit in the $j$th trace $t_j$ changes the estimator by at most
	\begin{align}
	    b & \leq  \frac{1}{T} \frac{1}{(1-p)^k}\left( \min(k, n-k+1) + \sum_{i = k+1}^d 2 \min(i, n-i+1) \max_{y \in Y_i (x)} \binom{y[2:i-1]}{x[2:k-1]} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + \sum_{i = k+1}^d 2 i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 d \max_{i \in [k+1, d]} i  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^k}\left( k + 2 d^2 \max_{i \in [k+1, d]}  \binom{i-2}{k-2} \left(\frac{p}{1-p}\right)^{i-k}\right)
	\end{align}
	To analyze $b$ when $k = c \log(n)$ for $c$ constant, and $p < 0.5$ we have that
    \begin{align} b & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 d^2 \max_{i \in [c\log(n)+1, d]}  \binom{i-2}{c\log(n)-2} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & \leq \frac{1}{T} \frac{1}{(1-p)^{c\log(n)}}\left( c\log(n) + 2 d^2 \max_{i \in [c\log(n)+1, d]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i-c\log(n)}\right)
    \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2d^2 n^{c \log(\frac{1-p}{p})}  \max_{i \in [c\log(n)+1, d]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}\right).
	\end{align}
	where we take $\log()$ to have base 2. 
	We have that
	\begin{align}
	    & \max_{i \in [c\log(n)+1, n]}  \binom{i}{c\log(n)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq \max_{i \in [c\log(n)+1, n]} 2^{i H(c\log(n)/i)} \left(\frac{p}{1-p}\right)^{i}
	    \\ & \leq 2^{ \frac{\log(n^c)}{1- p/(1-p)} H(1- p/(1-p))} \left(\frac{p}{1-p}\right)^{\frac{\log(n)} {1 - p/(1-p)}}
	    \\ & = n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} 
	\end{align}
	The maximizer is given by $i = \frac{\log(n^c)}{1- p/(1-p)}$ .
	This is because $x = \frac{\log(n^c)}{1- q}$ is the only zero of
	\begin{align}
	    & \frac{d}{dx} 2^{x H(c\log(n)/x)} q^{x} \\ & = q^x 2^{\log(n^c) (\log(1 - \log(n^c)/x) - \log(\log(n^c)/x)) - x \log(1 - \log(n^c)/x)} (\log(q) - \log(1 - \log(n^c)/x)), 
	\end{align}
	where $q = p/(1-p)$,
	the function is a differentiable for $x \in (c\log(n)+1, n),$
	and the second derivative of the function at $x = \frac{\log(n^c)}{1- q}$ is given by 
	\begin{align}
        - \frac{\log(n^c) (1-q) 2^{\log(n^c) \log(q)/(q-1) + \log(n^c)(\log(q) - \log(1-q))} q^{\log(n^c) / (1-q)}}{\log(n^c) (\log(n^c)/(1-q) - \log(n^c))}
	\end{align}
    which is negative.
    We therefore have that 
        \begin{align} b &
        \leq  \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{c \log((1-p)/p)}  n^{\frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
        \\ & = \frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}} \right)
	\end{align}    
    when $k = c\log(n)$ for $c$ constant and $p < 0.5$.
    Let
    \begin{align}
        f(p) = c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}
    \end{align}
	Plugging this into McDiarmid's inequality, and setting $\epsilon = 1/5$,  we have
	\begin{align}
		\Pr \left(\hat{N}_x - N_x \geq \frac{1}{5} \right) & \leq \exp \left(-\frac{2\left( \frac{1}{5}\right)^2}{nT  \left(\frac{1}{T} \frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right) \right)^2}\right)
		\\ & = \exp \left(-\frac{T}{\frac{25}{2}n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2}\right)
    \end{align}
    Setting $\delta = \Pr \left(\hat{N}_x - N_x \geq \frac{1}{5} \right)$, we have
    \begin{align}
        T = \log(1/\delta) \frac{25}{2} n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2
    \end{align}
    traces suffices for recovering $N_x$ with probability at least $1 - \delta$.

\subsection{comparison}

The number of traces needed to recover $N_x$ with probability at least $1- \delta$ for $p < 1/2$ using the truncated estimator is
\begin{align}
    & \log(1/\delta) \frac{25}{2} n \left(\frac{1}{n^{c\log(1-p)}}\left( c\log(n) + 2 d^2 n^{f(p)}  \right)\right)^2
    \\ & = O \left(d^4 n^{1 + 2 \left(f(p) + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
\end{align}
traces where
\begin{align}
    f(p) & = c \log((1-p)/p) + \frac{c H(1- p/(1-p))}{1- p/(1-p)} + \frac{\log(p/(1-p))}{1 - p/(1-p)}.
\end{align}
Observe that we can upper bound $f(p)$ as follows
\begin{align}
    f(p)  \leq c \log((1-p)/p) + \frac{c }{1- p/(1-p)}
\end{align}
by using the fact that $H(x) \leq 1$ for all $x$ and $\log(p/(1-p)) < 0$ for $p < 0.5$. 
Thus, the number of traces needed by our algorithm is upper bounded by 
\begin{align}
    & O \left(d^4 n^{1 + 2 \left(c \log((1-p)/p) + \frac{c }{1- p/(1-p)} + c\log\left(\frac{1}{1-p}\right) \right)}\right)\log(1/\delta) 
    \\ & = O\left(d^4 n^{1 + 2 c \log((1-p)/p) + \frac{2c }{1- p/(1-p)} + 2c\log\left(\frac{1}{1-p}\right)}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c (\log(1/p) + \frac{1 }{1- p/(1-p)})}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c (\log(1/p) + \frac{1-p}{1-2p})}  \right)\log(1/\delta)
    \\ & = O\left(d^4 n^{1 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)\log(1/\delta)
    \\ & = 	 O\left(log^4(n) \cdot n^{1 + 2 c \left(\log(1/p) + \frac{1/2-p/2}{1/2-p}\right)}  \right)
    \\ & = 	 O\left(log^4(n) \cdot n^{1 +  c \frac{1-p}{1/2-p} + 2c\log(1/p)}  \right).
\end{align}
Recall that the exponent of $n$ in the number of traces used by Servedio's algorithm is 
\al{4 + 12c \left(\frac{e^2}{1/2 - p}\right)    + c\log(4).}
Clearly, the number of traces used by our algorithm is smaller for $p$ close to $0.5$ and $c=1$ which is the $c$ they used in their paper.


